A Case for Sampling Based Learning Techniques in Coflow Scheduling

Coflow scheduling improves data-intensive application performance by improving their networking performance. State-of-the-art online coflow schedulers in essence approximate the classic Shortest-Job-First (SJF) scheduling by learning the coflow size online. In particular, they use multiple priority queues to simultaneously accomplish two goals: to sieve long coflows from short coflows, and to schedule short coflows with high priorities. Such a mechanism pays high overhead in learning the coflow size: moving a large coflow across the queues delays small and other large coflows, and moving similar-sized coflows across the queues results in inadvertent round-robin scheduling. We propose Philae, a new online coflow scheduler that exploits the spatial dimension of coflows, i.e., a coflow has many flows, to drastically reduce the overhead of coflow size learning. Philae pre-schedules sampled flows of each coflow and uses their sizes to estimate the average flow size of the coflow. It then resorts to Shortest Coflow First, where the notion of shortest is determined using the learned coflow sizes and coflow contention. We show that the sampling-based learning is robust to flow size skew and has the added benefit of much improved scalability from reduced coordinator-local agent interactions. Our evaluation using an Azure testbed, a publicly available production cluster trace from Facebook shows that compared to the prior art Aalo, Philae reduces the coflow completion time (CCT) in average (P90) cases by 1.50x (8.00x) on a 150-node testbed and 2.72x (9.78x) on a 900-node testbed. Evaluation using additional traces further demonstrates Philae's robustness to flow size skew.

==> Makefile <==
.SUFFIXES: .tex .dvi .ps .fig .eps .gnu .c
PDF = ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.2 -dSubsetFonts=true -dEmbedAllFonts=true
CFLAGS  =  -Wall -g -Os -march=i686 -mpreferred-stack-boundary=2 -I/usr/local/include
CC =	gcc
LDFLAGS = -lm
.c:
	$(CC) -o $@ $(CFLAGS) $< $(LDFLAGS)


#all: 	paper tr
#all: 	paper supp rebut
all: 	paper supp cleannonpaper cleanbib 

bib:	
	pdflatex paper
	bibtex paper
	#bibtex paper
	#pdflatex paper
#	pdflatex techreport
#	bibtex techreport 
#	bibtex techreport 
#	pdflatex techreport

paper: bib paper.tex
	pdflatex --shell-escape paper
	pdflatex paper
	mv paper.pdf ton.pdf

supp: supplementary.tex
	#pdflatex supplementary
	#bibtex supplementary
	pdflatex --shell-escape supplementary
	pdflatex supplementary

rebut: rebuttal-main.tex
#	pdflatex --shell-escape rebuttal-main 
#	pdflatex rebuttal-main

tr: techreport.tex
	pdflatex --shell-escape techreport
	pdflatex techreport
#	scp paper.pdf nescafe:~/Desktop/esys19-paper.pdf
#	gnome-open paper.pdf >out.out 2>err.err 

#	bibtex paper


#	dvips -Pdownload35 -t letter -o paper.ps paper.dvi
#	$(PDF) paper.ps

#	bash -c 'if [[ -f .Zheng ]]; then acroread paper.pdf; else ggv paper.ps; fi'
#	dvips -Pcmz  -t letter -o paper.ps paper.dvi
#	dvips -Pcmz  -t letter -o paper.ps paper.dvi
#	bibtex paper
#	sed -e 's/\(\\begin{thebibliography}{.*}\$\)/\1\\medskip/g' paper.bbl > paper.bbl.mv && mv paper.bbl.mv paper.bbl


sub:
	./submit.sh

aj: paper
	scp paper.pdf nescafe:~/Desktop/atc19-paper.pdf
	#scp paper.pdf nescafe:~/Desktop/esys19-paper.pdf
	#scp paper.pdf sp13:~/Desktop/CN18-paper.pdf
cleannonpaper:
	rm -rRf *.dvi *.aux *.blg *.log *.ps *~ *.out

cleanbib:
	rm -rRf *.bbl

clean: cleannonpaper cleanbib
	rm -rRf ton.pdf

cleanmajornonpaper: cleannonpaper
	rm -rrf *.out
cleanmajor: clean
	rm -rrf *.out
fresh : clean bib paper

freshaj : fresh aj 
	#scp paper.pdf nescafe:~/Desktop/CN18-paper.pdf
	#scp paper.pdf sp13:~/Desktop/CN18-paper.pdf
techreport: tr


==> Unix-LaTeX2e-Transactions-Style-File/IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> design.tex <==
\section{\name Design}
\label{sec:design}

%% \name is a novel coordinated coflow scheduling system which introduces
%% online coflow size learning into coflow scheduling. 
In this section, we present the detailed design of \name, which
%  The key objective in \name is to schedule coflows to \textit{reduce
%  the {average} CCT} without any prior knowledge of coflow
%  sizes. Additionally, \name aims to avoid starvation so that all
%  coflows can continually make progress.
addresses three design challenges:
(1) {\em Coflow size estimation:} How to choose and schedule the pilot flows for each newly arriving coflow?
(2) {\em Starvation avoidance:} How to schedule coflows after size estimation
using variations of SJF that avoid starvation?
(3) {\em \addtonreview{Inter-}coflow scheduling:} How to schedule among all the coflows with estimated sizes?
% (3) {\em Rate allocation:} How to allocate bandwidth among the flows at local ports?

%  We discuss the above three design components and how to tackle other challenges, like
%  starvation-freedom and work conservation.

\if 0
\iftoggle{tons}{
{\color{red}	%	closing bracket on line 64
\subsection{Additional Design Challenges}

\paragraph{Non-Clairvoyant Coflows.}
Traditional scheduling schemes virtually based on some characteristics
of the coflows. Under circumstances that these characteristics are
unknown a priori and provided that classic solutions Least-Attained
Service and its adaption to coflows have been proved inefficient, we
need new online algorithms that make efficient scheduling.

\paragraph{Real-time Decision.} 
The coordinator needs to make real-time decision in the given
synchronization cycle, and therefore, the scheduling algorithm should
not be of large time complexity. Previous heuristics such as
Smallest-Effective-Bottleneck-First and
Minimum-Allocation-for-Desired-Duration in
Varys~\cite{varys:sigcomm14}, Discretized Coflow-Aware Least-Attained
Service in Aalo~\cite{aalo:sigcomm15}, \etc, may fail to finish
computation in a small synchronization cycle.  In \name we aim to
provide a much simpler scheduling algorithm without recalculating
priority all the time.

\paragraph{Scalability.}
These heuristics need to either continuously recalculate priority of  coflows
between synchronization cycles or to exchange lots of messages between local
agents and  the global coordinator. In the evaluation of our testbed, these
drawbacks will bring large computation and communication overhead, and limit
the scalability of the scheduler.

\paragraph{Starvation Freedom.}
It sounds plausible that we  schedule the shortest coflow all the time. But
this may bring a common starvation problem. Assuming that there are always new
and preferable coflows entering the system, the largest coflow in the system,
though admitted for a very long time, will not receive any service and never
finish (aka. starve).  When designing the scheduler, we must assure that
however the workload is, every coflow will finish in a finite time.


\subsection{Scheduling Algorithm}
\name adopt \textit{Flow Probing} to estimate coflow size, \textit{Estimatedly
Shortest Job First} (ESJF) to define the priority of coflows, and
\textit{weighted sharing among multiple queues} to eliminate starvation and
retain fairness.
}}{}
\vspace{-0.1in}
\fi



\subsection{\name architecture}
\label{sec:design:arch}

Fig.~\ref{fig:design:arch} shows the \name architecture \name models
the entire datacenter as a single big-switch with each computing node as
an individual port. The scheduling function in \name is divided among \edittonreview{(1)
a central coordinator, and (2) local agents that run on individual
ports.}{ the following two entities: (1) a central coordinator - which is responsible for making decisions of flow priorities and sending rates, and (2) local agents that run on individual
ports - they are responsible for executing the coordinator's decision.}  A computing framework such as Spark~\cite{acm:spark} first
registers (removes) a coflow  \addtonreview{with the central coordinator} when a job arrives (finishes).
\addtonreview{The central coordinator functions in an event-driven manner: }
upon a new coflow arrival, old coflow completion, or pilot flow completion,
% based on the coflow information from the framework, and the estimation of coflow sizes
% (\S\ref{sec:design:pilot}), 
\edittonreview{the coordinator}{it} calculates a new 
coflow schedule\edittonreview{, which includes}{. The new schedule includes the following two pieces of information:} (1) coflows that are to be scheduled
in the next time slot, and (2) flow rates for the individual flows of a
coflow\edittonreview{, and}{. It then} pushes this information to the local agents which use
this information to allocate \edittonreview{their bandwidth}{bandwidth to each flow}. The local agents will
follow the current schedule until they receive a new schedule.

\begin{figure}[t]
  \centering
\vspace{-0.2in}
  \includegraphics[width=0.95\linewidth, natwidth=610,natheight=642, page = 3]{figs/arch-nsdi.pdf}
\vspace{-0.4in}
  \caption{\name architecture.
}
\vspace{-0.2in}
  \label{fig:design:arch}
\end{figure}

\vspace{-0.1in}
\subsection{Sampling pilot flows \addtonreview{for coflow-size estimation}}
\label{sec:design:pilot}

% In \name,  the coflow sizes are unknown apriori. 
As discussed in \S\ref{sec:key}, \name estimates the size of a coflow
online by actually scheduling a subset of its flows (\textit{pilot
  flows}) at their ports. We do not schedule the flows of a coflow
other than the pilot flows until the completion of the pilot flows in order to
avoid unnecessary extra blocking of other potentially shorter coflows.

\vspace{-0.05in}
\paragraph{How many pilot flows?} 
When a new coflow arrives, \name first needs to determine the number
of pilot flows. {{As 
%we briefly 
discussed at the end of \S\ref{sec:key}, the}} number of pilot flows affects the trade-off
between the coflow size estimation accuracy and  scheduling overhead.
For coflows with skewed flow sizes,
accurately estimating the total coflow size potentially requires
sampling the sizes of many pilot flows. However, scheduling pilot flows has associated
overhead, \ie if the coflow turns out to be a large coflow and should have been 
scheduled to run later under SJF.
%  Since the global coordinator prioritizes pilot flows over other
%  flows on the ports where the pilot flows are scheduled,
%  scheduling pilot flows essentially pushes back flows of other coflows
%  on the same ports, thus elongating CCT of those coflows.

%% At one extreme, simply
%% selecting a single pilot flow results in poor accuracy but has the
%% least overhead. At the other extreme, selecting all flows will have a
%% perfect accuracy but incur high overhead at the same time.

We explore several design options for choosing the number of pilot flow.
Two {natural} design choices are
using a {constant number of pilot flows} or a
fixed fraction of the total number of flows of a coflow. In addition, we
observe that typical coflows consist of flows between a set of senders (\eg
mappers) and a set of receivers (\eg reducers)~\cite{mapreduce:osdi04}.
% and the flows from a single sender (\eg a mapper) to multiple receivers have
% the same size~\cite{mapreduce:osdi04}.  \commentaj{I don't think that the
% above claim is correct. ~\cite{mapreduce:osdi04} says that input to each
% mapper is of equal size. However it doesn't say that flows from a single
% sender to multiple receivers have the same size. This flaw was highlighted in
% NSDI review too. Maybe we can say that input to each mapper is of equal size
% and they run the same program so it is likely that output of mappers in
% general will be similar?} \editaj{and the input to each mapper tends to be of
% equal size and the mapper tasks run the same program and thus it is likely
% that their output will be of similar sizes.}{}
%
We thus include a third design choice of a fixed fraction of sending
ports. {This design also spreads the pilot flows to avoid
having multiple pilot flows contending for the same sending ports.}
% mappers to avoid multiple pilot flows scheduled on the same mapper port that
% causes contention and elongates the completion of pilot flows as well as rest
% of the flows on those ports.
We empirically found that
(\S\ref{sec:sim:probeOverhead}) limiting the pilot flows to 5\% to 10\% of the
number of its sending ports (\eg mappers in a MapReduce coflow) strikes a good
balance between estimation accuracy and overhead. {We note the total number of flows
sampled in this case is still under 1\%.
}
%  \comment{However, there are some works like LEEN\cite{LEEN:CLOUDCOM2010} and
%  Mantri\cite{mantri:OSDI2010} that have highlighted the problem of skew in multi
%  phase distributed jobs. So, we derived a trace which matches the skew described
%  in \cite{mantri:OSDI2010} and we observed that \name was performing similar on
%  the skewed trace too (fig. \ref{fig:sim:skewedTrace}).}

Finally, we \textit{estimate the total coflow size as $S = f_i \cdot N$}, where
$N$ is the {number of flows in a coflow, and $f_i$ is the average size
 of the sampled pilot flows.}

%{total number of flows of the coflow that have started so far, and \name updates
%the estimated size when some new flows start. $f_i$ is the average size of the
%sampled pilot flows.}

%\addaj{(value of $N$ can be calculated as product of number of senders and receivers.)}
\vspace{-0.05in}
\paragraph{Which flows to probe?}
Second, \name needs to decide which ports to schedule the chosen number of probe
flows for a coflow. For this, we use a simple heuristic where, upon the arrival
of a new coflow, we select the ports for its pilot flows that are least busy,
\ie having pilot flows from the least number of other coflows. \name
starts with the least busy sending port and iterates over receiving ports
starting with the least busy receiving port and assigns the flow if it exists \addtonreview{\footnote{\addtonreview{Note that Philae chooses the least busy ports for sampling. This conditioning has very little impact on the distribution of the size of the sampled flows because flow sizes have no relation to the sending or receiving port. Hence, Philae’s sampling of flows can be viewed as independent.}}}. It
then updates the statistics for the number of pilot flows scheduled at each port and
repeats the above process. Such a choice
will likely delay fewer coflows when the pilot flows are scheduled
and hence reduce the elongation on their CCT.
%  \addaj{Though there is a possibility that no flow of the coflow at one of
%  least-contentious ports is ready to be scheduled. In such case \name
%  coordinator can simply move to a next port in order of increasing contention.}
We note that such an online heuristic may not be optimal; more sophisticated
algorithms can be derived by picking ports for multiple coflows together.
However, we make this design choice for its simplicity and low time complexity
to ensure that the coordinator makes fast decisions.

\vspace{-0.05in}
\paragraph{How to schedule pilot flows?}
In \name, we prioritize the pilot flows of a new coflow over existing
flows to accelerate learning the size of the new coflow.
In particular, at each port, pilot flows have high priority over
non-pilot flows. If there are multiple outstanding pilot flows (of different
coflows) at a port, \name schedules them in the FIFO order.

\vspace{-0.1in}
\subsection{Coflow scheduling with starvation avoidance}
\label{sec:design:starvation}

\if 0
Once the coflow sizes are estimated, the natural way of scheduling coflows is
to use shortest- or smallest- job first (SJF) (or their variations) because of
their known optimality. In SJF, the coflows are scheduled in the increasing
order of their sizes. 
% {We should not say this that natural way is SJF? Because in Varys and Saath people have already reported that SJF on size in not the optimal way. A reviewer also said similar thing in NSDI 18 review. I am not sure how to change here. Can you help?}
% { I added known variations. what did these papers criticize about SJF here?}
% {Varys says that SJF doesn't take width of a coflow into account and it can also be influenced by one single large flow. In SAATH the authors have said that SJF doesn't account for contention}
Alternatively, \name can use Shortest-Effective-Bottleneck first (SEBF) in
Varys~\cite{varys:sigcomm14}, which assumes known coflow size and width. 
%  SEBF schedules coflows in the increasing order of the expected
%  CCT, calculated based on flow lengths and bandwidths available at
%  individual ports. 
However, neither approach accounts for starvation
avoidance -- an intrinsic drawback of any SJF-like online schemes.
%  , where a
%  coflow at the end of the queue can wait indefinitely with continuous
%  arrival of new shorter coflows.
\fi

Once the sizes of coflows are learned, we can apply variations of the
SJF policy to schedule them.  However, it is well known that such
policies can lead to starvation. 

There are many ways to mitigate the starvation issue. However, a
subtlety arises where {\em even slight difference in how starvation is
addressed can result in different performance}. For example, the
multiple priority queues in Aalo has the benefit of ensuring progress
of all coflows, but assigning different time-quanta to different
priority queues can result in different average CCT for the same
workload.
To ensure the fairness of performance comparison with Aalo,
we need to ensure that both \name and Aalo provide the same level of
starvation freedom (or progress measure).

For this reason, in this paper, we inherit the
multiple priority queue structure from Aalo for coflow scheduling.
As in Aalo, \name sorts the coflows among multiple priority queues. 
In particular, \name uses $N$ queues, $Q_0$ to
$Q_{N-1}$, with each queue having lower queue threshold Q$^{lo}_{q}$
and higher threshold Q$^{hi}_{q}$, where Q$^{lo}_0$ = 0, Q$^{hi}_{N-1}$
= $\infty$, Q$^{lo}_{q+1}$ = Q$^{hi}_{q}$,
and the queue thresholds grow exponentially, \ie Q$^{hi}_{q+1}$ = E
$\cdot$ Q$^{hi}_{q}$.
%\name uses exponentially growing queue thresholds, \ie Q$^{hi}_{q+1}$ = E
%$\cdot$ Q$^{hi}_{q}$.
%   By default, \name sets E = 10, K = 10, shown to be
%   effective in our evaluation (\S\ref{sec:sim:sa}).

The overall coflow scheduling in \name works as follows.
After the coflow size is estimated using pilot
flows, \name assigns the coflow to the priority queue using
inter-coflow policies discussed in \S\ref{sec:design:intercoflow}.
Within a queue, we use FIFO to schedule coflows. Lastly, we use
weighted sharing of network bandwidth among the queues, where a
priority queue receives a network bandwidth based on its priority. 
As in Aalo, the weights decrease exponentially
% (with a factor of 10)
with decrease in the priority of the queues.

Using FIFO within the priority queue and weighted fair sharing among
the queues together ensure the same starvation freedom and thus meaningful
performance comparison between \name and
Aalo~\cite{aalo:sigcomm15}.

%\vspace{-0.1in}
\subsection{Inter-coflow scheduling policies}
\label{sec:design:intercoflow}

%  Shortest job or remaining time first heuristics are shown to be
%  optimal when minimizing average execution time when execution depends
%  on single resource (\eg processes in single-CPU system or flows on a
%  single link). Naturally, coflows can be scheduled using
%  Shortest (or Smallest) coflow First. However, such scheduling can be
%  suboptimal as it ignores \textit{contention} of the coflow, \ie the
%  number of other coflows blocked on its multiple ports, which can vary
%  at different ports~\cite{jajooSaath}. Effectively, when a coflow is scheduled, the
%  increase in the waiting time of other coflows depends on the coflow
%  size as well as the {\em contention} caused by scheduling individual
%  flows at individual ports. 
%  Formally, the contention of scheduling a
% flow $i$ at port $j$ is defined as the number of coflows blocked at
% port $j$.

\if 0
In \name, we explore four different scheduling policies based on different
combinations of coflow size and contention, as summarized in
Table~\ref{algo:inter-coflow}: 2 size-based policies (\textit{A, B}) and
{1 contention-based, similar to what is used in \cite{jajooSaath} (\textit{C}), and
a contention-and-length-based policy (\textit{D})}. For all four
policies, we continue to use the priority-queue based scheduling, and the
policies only differ in what metrics they use in assigning coflows to the
priority queues.
\fi

%In \name, we explore six different scheduling policies based on different
%combinations of coflow size and contention, as summarized in
%further: 2 size-based algorithms (\textit{A, B}) and
%{1 contention-based, similar to what is used in \cite{jajooSaath} (\textit{C}), and
%3 contention-and-length-based algorithms (\textit{D, E, F})}. For all six
%algorithms, we continue to use the priority-queue based scheduling, and the
%algorithms only differ on what metric they use in assigning coflows to the
%priority queues.
In \name, we explore six different scheduling policies based on different
combinations of coflow size and contention,
% as summarized
% {Removing the table helps in saving the space}
%{in Table~\ref{algo:inter-coflow}}{further}:
two size-based policies (\textit{A, B}) as in Aalo,
{a contention-based, similar to the intra-queue policy used in Saath~\cite{jajooSaath} (\textit{C}), and
three new contention-and-length-based policy (\textit{D, E and F})}:

We use the following parameters of a coflow to define the metrics in
\edittonreview{scheduling algorithms}{the above scheduling policies}:
(1) average flow length ($l$) from piloting, 
{(2) number of flows ($n$), 
(3) number of sender and receiver ports ($s, r$),}
%{
%(2) number of sender and receiver ports ($s, r$)\footnote{{\name only needs to know the number of ports and not the location of the nodes.}},
%(3) number of flows ($n$), 
%}
(4) total amount of data sent so far ($d$),
(5) contention ($c$), defined as the number of other coflows sharing
any ports with the given coflow, and
(6) port-wise contention ($c^p$), defined as the number of other coflows
blocked at a given port $p$.

%\begin{description}[noitemsep,topsep=0pt,leftmargin=0.2in]
%\vspace{-0.1in}
{\bf (A) Smallest job first:} Coflows are sorted based on
  coflow size ($l \cdot n$).

{\bf (B) Smallest remaining data first:} Coflows are sorted
  based on remaining data ($l \cdot n - d$).

{\bf (C) Least global contention first:} Coflows are sorted based on
  their global contention ($c$).

{\bf (D) Least length-weighted total-port contention first:} Coflows are sorted
based on the sum of port-wise contention times estimated flow
length $\sum \limits_{p}c^p \cdot l$.

\iftoggle{tons}{
{%\color{red}	%	closing bracket on line 348

{\bf (E) Least length-weighted max-port contention first:}  Coflows are sorted based
on the maximum waiting time increase across ports
$\max \limits_{p}c^p\cdot l$.

{\bf (F) Least length-weighted contention first:} Coflows are sorted based
on the product of global contention and length ($c \cdot l$). This metric is
indicative of average waiting time increase across ports.
}
}{}
%\end{description}




\name uses Policy D by default, % least total-port contention first,
as it results in the least average CCT (\S\ref{sec:sim}).
For all policies, we continue to use the priority-queue based
scheduling, and the algorithms only differ in what metric they use in
assigning coflows to the priority queues.
In contrast, Aalo does not handle inter-coflow contention, and uses
the total bytes sent so far ($d$) to move coflows across multiple priority
queues.
% \ajadd{Following are six(6) scheduling policies we explored:}
%% further develops the idea of contention with calculating the total
%% contending time one coflow introduces at a port level instead of the
%% whole network.  We define the novel \textit{port-wise contention} as
%% \textit{the number of coflows this job is blocking at one port}.  For
%% each port the coflow is sending data at, we calculate a port-wise
%% impact $I^p = C^p * LN$ . \textit{E} and \textit{F} respectively take
%% the maximum and sum of all port-wise impacts.  \eg $I_E = \max
%% \limits_{p}I^p$, $I_F = \sum \limits_{p}I^p$
\input rate_alloc
%   \addaj{However, since \name tries to schedule only one pilot flow of a coflow
%   at a port, hence bandwidth assigned to a pilot flows is $min(B(s),B(r))$ and
%   they do not share bandwidth with other flows of the parent coflow at same
%   port.}
%\paragraph{\name algorithm}
% \input algo

%% As we analyzed in Section %\ref{sec:keyidea}
%% , we can estimate the total size of a coflow by first scheduling some (at least one) selected flows as probes. These flows are called \textit{pilot flows}. By carefully selecting pilot flows,  we can get extraordinary accuracy of total size while bringing very little overhead. Before the probing stage finishes, the coflows are called \textit{teenager coflows} and they are placed in the \textit{teenager queue}. To make probing stage finish as soon as possible to efficiently determine the priority, pilot flows of the teenager coflows have the highest priority to be scheduled.

%% Those coflows whose pilot flows have been finished are designated as \textit{adult coflows}. At the time when a teenager coflow get mature (finish all its pilot flows), the scheduler calculate its estimated size, based on which the coflow is plugged  into one of the \textit{adult queues}. To implement \textit{Estimatedly Shortest Job First} while retaining starvation freedom, we adopt a weighted sharing among adult queues structure. Adult queues containing \textbf{smaller} coflows have \textbf{more} proportion of time for better performance, while those containing \textbf{larger} coflows have \textbf{less} time just for liveness. Inside each queue, the scheduler adopt the \textit{First In First Out} (FIFO) order to schedule coflows in that queue for starvation freedom.

%% To help readers gain a better understanding of the workflow of the scheduler, the life cycle of a coflow is illustrated in Figure \ref{fig:lifecycle} and the pseudocode of setting rates is shown below.

%% %\if 0

\vspace{-0.1in}
\subsection{Additional design issues}
\label{sec:design:additional}


\paragraph{Thin coflow bypass.}
Recall that, in \name, when a new coflow arrives, \name only schedules
its pilot flows. All other flows of that coflow are delayed until the
pilot flows finish and coflow size is known. However, such a design
choice can inadvertently lead to higher CCTs for coflows, particularly
for thin coflows, \eg a two-flow coflow would end up serializing 
scheduling its two flows, one for the piloting purpose.

\if 0
%  To minimize the overall CCT, a short coflow should be scheduled
%  immediately. However, when pilot flows of such coflows are scheduled,
%  the other flows have to wait till the completion of the pilot flows,
%  which delays their completion, and increases their CCT as well as
%  overall.
Fig.~\ref{fig:sim:designComponent:thinNeed} shows that by
default the ratio of piloting time to the total time is surprisingly
high for those thin coflows (width $\leq$ 7) while virtually
negligible for those wide coflows (width $>$ 10).

\begin{figure}[t]
\centering
\includegraphics[width=0.85\linewidth]{figs/ProbingPortion_numFlows.eps}
\caption{Cost of piloting in \name: 
the fraction of CCT spent in piloting as a function of the coflow width.
\updated{05/26/2018}
}
\label{fig:sim:designComponent:thinNeed}
\end{figure}
\fi

%  Similar to Graviton~\cite{graviton:hotcloud16}, we use width as an
%  indicator to coflow size. Coflows with smaller width tend to have
%  smaller size.
To avoid CCT degradations for thin coflows, we schedule all flows
of a coflow if its width is under a threshold (set to 7 in \name;
\S\ref{sec:sim:sa} provides sensitivity analysis for 
thresholds).

\paragraph{Failure tolerance and recovery.}
Cluster dynamics such as stragglers or node failure can delay some of
the flows of a coflow or start new flows, increasing their CCT. The \name design
automatically self-adjusts to speed up coflows that are affected
by cluster dynamics using the following mechanisms: (1) It adjusts
the coflow size as the amount of data left by the coflow, which is
essentially the difference between the size calculated using pilot
flows and amount of data already sent. (2) It calculates contention
only on the ports that have unfinished flows.
%  Based on these updates,
%  the global coordinator then changes the priority queue of a coflow.  

%% \commentrg{People are going to ask on how to choose the threshold.}

\paragraph{Work Conservation.}
By default, \name schedules non-pilot flows of a coflow only after all its pilot flows
are over. This can lead to some ports being idle where the non-pilot flows are waiting for the pilot flows to finish.
%  However, it is possible that some ports do not have flows of a thin coflow
%   or a coflow whose sampling phase is over ready to send.
In such cases, \name schedules non-pilot flows of coflows which are
still in the sampling phase at those ports. In work conservation, the coflows are
scheduled in the FIFO order of {arrival of} coflows.

==> discussion.tex <==
\section{Discussions}
\label{sec:dis}

\if 0
\paragraph{DAG workloads (chain among jobs):} 
Often times a single analytics query contains multiple
co-dependent stages with each stage containing multiple analytics
jobs. Such queries are usually represented as a Directed Acyclic Graph
(DAG) to capture the dependencies (\eg Hive~\cite{hive:web}) between
the stages. The completion of a stage depends on the completion of the
last job in that stage, whereas completion of the query depends on the
completion of the last stage. Na\"{\i}vely, each job can be sped up by
representing it with a single coflow, and then speeding up the coflows
(\S\ref{sec:design}). However, instead of representing a single job
with single coflow, we represent each individual \textit{stage} with a
different coflow. Such optimization helps \name to slow some of the
fast jobs in one stage without slowing down that stage.
\fi

\paragraph{Generalizing the idea of probing} 
The key idea of pre-scheduling sampled flows can be generalized to
other job scheduling in distributed settings. For example, in cluster job
scheduling, a subset of the tasks of a job can be scheduled on some of
the least busy VMs to gather more information about the CPU, memory
usage and output data volume (instead of learning from
history~\cite{corral:sigcomm15}), which can be used for efficiently
scheduling the remaining tasks (\eg using SJF).

\if 0
\paragraph{Failure tolerance and recovery}
Cluster dynamics such as node failure or stragglers can delay some of
the flows of a coflow, increasing their CCT. The current \name design
automatically self-adjusts to speed up coflows that are slowed down
due to cluster dynamics using the following mechanisms: (1) We adjust
the coflow size as the amount of data left by the coflow, which is
essentially the difference between the size calculated using pilot
flows and amount of data already sent. (2) We calculate contention
only on the ports that have unfinished flows. Based on these updates,
the global coordinator then changes the priority queue of a coflow.
\fi

\paragraph{Buffering overhead} may seem like a concern for \name as non-piloted
flows of a coflow need to be buffered at the sending ports.  However, buffering
is actually common to all coflow scheduling policies, \eg arrived coflows are
also buffered at the sending ports in Aalo as they move across the priority
queues.  Since \name provides better average CCT, the average buffer delay of
coflows is lower than other polices.
% We measure the total data accumulated across all the ports every 8ms and
% $Average(90^{th})$ percentile for \name is 9.73 TB(27.1 TB) and so is for
% Aalo.
  We omit detailed measurment due to space limitation.


\addaj{
\paragraph{Security Issues:} \name's approach of giving high priority to pilot flows might also expose a vulnerability for denial of service attack at some ports. The multiple priority queue structure helps countering the problem.
}
  


==> intro.tex <==
\vspace{-0.2in}
\section{Introduction}
\label{sec:intro}

\subsection{Motivation}
\label{sec:intro:moti}
In big data analytics jobs, speeding up the communication stage \addtonreview{(}where
the data is transferred between compute nodes\addtonreview{)} is important to speed up
the jobs. However, improving network level metrics such as flow
completion time may not translate into improvements at the application
level metrics such as job completion time. The coflow
abstraction~\cite{coflow:hotnets12} was proposed to bridge such a
gap. The abstraction captures the collective network requirements of
applications, as reduced coflow completion time (CCT) can directly
lead to faster job completion time~\cite{orchestra:sigcomm11,baraat:sigcomm14}.

%  which is then used to improve the network level
%  performance that directly translates into application
%  performance improvements.

%  However, inter-coflow scheduling to minimize the average coflow completion time (CCT)
%  is known to be NP-hard~\cite{varys:sigcomm14}. 
There have been a number of efforts on network designs for
coflows~\cite{varys:sigcomm14, sunflow:conext16, sincronia:sigcomm18} that
assume complete prior knowledge of coflow
% {characteristics such as the number of flows and their}
sizes (The coflow size is defined as the total size of its constituent
flows.).  However, in many practical settings, coflow characteristics are not
known a priori. For example, multi-stage jobs pipeline data from one stage to
the next as soon as the data is generated, which makes it difficult to know the
size of each flow~\cite{plausibleFlowSize, mapreduceonline:nsdi2010}.
A recent study~\cite{plausibleFlowSize} shows various other reasons
why it is not very plausible to learn flow sizes from applications, for
example, learning flow sizes from applications requires changing either the
network stack or the applications.

Scheduling coflows in such {\em non-clairvoyant} settings, however, is
challenging. The major challenge in developing an effective
non-clairvoyant coflow scheduling scheme has centered around how to
learn the coflow sizes online quickly and accurately, as once the
coflow sizes (bytes to be transferred) can be estimated, one can
apply variations of the classic Shortest-Job-First (SJF) algorithm
such as Shortest Coflow First~\cite{varys:sigcomm14} or apply an LP
solver (\eg \cite{sincronia:sigcomm18}).
% , where the coflow job length is loosely defined as the total bytes of the coflow, \ie of all its
% flows.
%  However, using SCF \textit{online} is not practical as it
%  requires prior knowledge about the coflow sizes. This is further
%  complicated as coflows arrive and exit dynamically and by cluster
%  dynamics such as failures and stragglers.
%
% {\cite{varys:sigcomm14} doesn't use SJF.
% It is using SEBF} {is SEBF a variant of SJF?}
% { SEBF is trying to schedule in shortest-Impact-first order. Its goal is to minimize the
% opportunity(for other coflows) lost in scheding each coflow. It takes length,
% width, size, and skew into account.}.

State-of-the-art online non-clairvoyant schedulers such as
Saath~\cite{jajooSaath}, Graviton~\cite{graviton:hotcloud16} and
Aalo~\cite{aalo:sigcomm15}  
\edittonreview{in essence learn coflow sizes and approximate SJF}{try to approximate SCF (inspired by SJF scheduling in single-server queues, which is known to minimize the average completion time of tasks). They implement this idea}
using discrete priority queues, where all newly arriving coflows start from the
highest priority queue, and move to lower priority queue as they send more data
(without finishing), \ie cross the per-queue thresholds.
% In particular, it starts a newly arrived coflow in the highest
% priority queue and gradually moves it to the lower priority queues as
% the total data sent by the coflow exceeds the per-queue thresholds.
In this way, the smaller coflows finish in high priority queues, while
the larger coflows gradually move to the lower priority queues where
they finish after smaller coflows.


%   The key idea in Aalo is to approximate SCF by learning coflow length
%   using {discrete priority queues}.
% by transitioning the coflows across the queues using the total
% bytes sent so far by a coflow.
%  The above idea is generic and applicable to scheduling
%  sequential jobs (\eg single flows) on a single work engine (\eg a
%  single network port). 
To realize the above idea in scheduling coflows which have
flows at many network ports, \ie in a distributed setting, Aalo uses a
global coordinator to assign coflows to logical priority queues, and
uses the total bytes sent by all flows of a coflow as its logical
``length'' in moving coflows across the queues.
The logical priority queues are mapped to local priority queues at each port,
and the individual
local ports then schedule the flows in its local
priority queues, \eg by enumerating flows from the highest to lowest
priority queues and using FIFO to order the flows within each queue.

In essence, Aalo learns coflow sizes by actually scheduling the
coflow, a ``try and miss'' approach to approximate SJF. As coflow
sizes are not known, in each queue, Aalo schedules each coflow for a
fixed amount of data (try).
% in the hope that the coflow finishes in that queue.
If the coflow does not finish (miss), it is demoted to a
lower priority queue. Afterwards, such a coflow will no longer block
coflows in higher priority queues.

\if 0
Generally speaking, using multiple priority queues in Aalo in this way
has three effects: (1) {\bf Coflow segregation:} It segregates long
coflows (who will move to low priority queues) from short coflows who
will finish while in high priority queues; (2) {\bf Finishing short
  coflows sooner:} Since high priority queues receive more bandwidth
allocation, short coflows will finish sooner (than longer ones); (3)
{\bf Starvation avoidance:} Using the FIFO policy for intra-queue
scheduling provides starvation avoidance, since at every scheduling
slot, each queue at each port receives a fixed bandwidth allocation
and FIFO ensures every coflow (its flow) in each queue is never moved
back.
\fi

Using multiple priority queues to learn the relative coflow sizes of
coflows this way, however, negatively affects the average CCT and the
scalability of the coordinator:

\textbf{(1) Intrinsic queue-transit overhead:} Every coflow that Aalo transits
through the queues before reaching its final queue worsens the average CCT because
during transitions, such a coflow effectively {\em blocks other shorter} coflows in the
earlier queues it went through, which would have been scheduled before this coflow starts in a
perfect SJF.
% , worsening their CCT.

%% This negative effect is further amplified as the time a coflow spends
%% in each queue grows exponentially with the queues, which translates
%% into an exponential increase in the CCT of the blocked coflows.

\textbf{(2) Overhead due to inadvertent round-robin:} Although Aalo
attempts to approximate SJF, it inadvertently ends up doing
{\em round-robin} for {coflows of similar sizes} as it moves them across
queues. Aalo assigns a \textit{fixed threshold of data transfer} for
each coflow in each queue. Assume there are ``$N$'' coflows in a queue
that do not finish in that queue. Aalo schedules one coflow (chosen
using FIFO) and demotes it to a lower priority queue when the coflow
reaches the data threshold. At that point, the next coflow from the
same queue is scheduled, which joins the previous coflow at a lower
priority queue after exhausting its quantum, and this cycle continues
as coflows of similar sizes move through the queues. Effectively, these
coflows experience the round-robin scheduling which is known to have
the worst average {CCT}~\cite{OSConcepts},
when jobs are of similar sizes.

\if 0
\textbf{(3) Overhead in scheduling all flows:} To learn the coflow sizes,
when a coflow arrives, Aalo schedules \textit{all} its flows at all
their ports. This replicates and hence amplifies the above intrinsic
queue-transit overhead and round-robin overhead at all those ports.
\fi

\textbf{(3) Limited scalability from frequent updates from local ports:} To support the try-and-error
style learning, the coordinator requires frequent updates from all
local ports of the bytes sent for each coflow in order to move coflows
across multiple queues timely. This results in high load on the
central coordinator from receiving frequent updates and calculating and
sending new rate allocations, which limits the scalability of the overall approach.

\if 0
Intuitively, the {\em learning overhead} of a coflow C1, defined as
the portion of the bytes that has been transferred (or the fraction of
its CCT spent in doing so) before reaching its correct queue, directly
translates into the delay incurred on any other coflow C2 that was
``shorter'' or ``of same size'' but did not finish until after the
learning of coflow C1 completed. In other words, if an oracle told us
that C2 was shorter than or of the same size as C1 when C1 first
arrived, we could have allocated all the bandwidth resources used for
learning C1 before C2 finishes to C2, so C2 would finish sooner,
without affecting the completion time of C1.\footnote{This is the same
swapping argument in the optimality proof of SJF.}
\fi


\paragraph{Empirical measurement}
%
We quantify the coflow size {\em learning overhead}
of Aalo, defined as
the portion of the bytes of a coflow that has been transferred (or the fraction of
its CCT spent in doing so) before reaching its correct queue,
using a trace from Facebook clusters~\cite{fbtrace:web} (see detailed methodology
in \S\ref{sec:sim}).
% We define the {\em learning overhead} as the time
% a coflow spent before reaching the correct (final) priority queue as a fraction of its CCT.
% that were transmitted at all the ports where it has flows before the
% global coordinator moves it to the final ``correct'' queue.
% \ie the final actual queue at all its ports.
Figure~\ref{fig:sim:learningCost} shows that ~40\% of the coflows that moved beyond
the initial queue reached the correct priority queue after spending more than
20\% of their CCT moving across early queues.
%Figure~\ref{fig:sim:learningCost} shows that 62.5\% of the coflows that moved beyond
%the initial queue reached the correct priority queue after spending more than
%22\% of their CCT moving across early queues.
% {Here we are defining bytes used as learning overhead but the figure~\ref{fig:sm:learningCost} is about time and also says same in the caption}
\begin{figure}[tp]
\centering
%	\subfigure[CDF of ratio of estimated size and actual size of coflows.]
  \includegraphics[width=1.0\linewidth,natwidth=610,natheight=642]{figs/ProbingPortion.pdf} %done
%  \includegraphics[width=\textwidth]{figs/ProbingPortion.eps} %done
% \caption{\name accuracy and overhead }
\vspace{-0.3in}
\caption{CDF of learning overhead per coflow, \ie
the time to reach the correct priority queue as a fraction of CCT, 
%  For \name, it is also the fraction of time spent in the probing phase
%  compared to the CCT. 
excluding coflows directly scheduled by \name or finish in Aalo's first queue.
%  \updated{06/11/2018}
}
\label{fig:sim:learningCost}
%\label{fig:sim:probingEffectiveness}
\vspace{-0.25in}
\end{figure}
%% This overhead also exists in the serial version of using multiple
%% queues to approximate SJF, where multiple jobs with unknown sizes
%% compete for a single resource.  In essence, any time a job consumes
%% the resource (\ie when scheduled to run) while in the queues other
%% than the final queue it belongs to (based on its size), it elongates
%% the average CCT.  This is manifested in two ways. (1) When two
%% similar-size (\eg large) jobs are sieved through the queues, they are
%% effectively interleaved, which leads to the worse average CCT, \ie
%% round-robin of two equal-size jobs. In other words, large jobs
%% elongate each other's CCT.  (2) When a small job $i$ belonging to
%% queue $i$\footnote{Queue 0 is the highest priority.} and a large job
%% $j$ belonging to queue $j>i$ are sieved through queues 0 to i, they
%% are effectively interleaved (\ie round-robin), which leads to longer
%% CCT for the small job compared to scheduling job $i$ first followed by
%% job $j$ (if their size were known).  In other words, the CCT of small
%% jobs are affected by large jobs.
%% \item[Overhead from moving all flows:]
%  Such penalty can be substantially
%  high, especially for the long coflows that move the queues
%  incrementally while spending exponentially more time and bandwidth at
%  each queue before reaching its final queue.
%% To learn the coflow size, when a coflow arrives, Aalo schedules
%% \textit{all} its flows at all their ports, \ie it moves flows across
%% queues at each of the coflow's ports, which amplifies the intrinsic
%% queue-sieving overhead at all those ports, elongating the the CCTs of
%% all affected coflows.
%% \end{description}
 \vspace{-0.15in} 
\subsection{Our Contribution}

We propose \name, a new non-clairvoyant coflow scheduler with a
dramatically different approach to learning coflow sizes to enable online SJF.
%  Like prior-art, \name is non-clairvoyant, \ie it does not require any prior
% knowledge, and also approximates Smallest Coflow First (SCF) derived from SJF.
%\addaj{\name uses number of sender and receiver tasks involved in a coflow
%to make scheduling decision. However, these decisions are indifferent to
%location of the tasks, information regarding number of tasks is available at
%the coordinator.} \questionaj{Should we also write anything about multi-wave here?}
To leverage optimal scheduling SJF in coflow
scheduling, it is vital to learn the coflow sizes quickly and accurately. \name
achieves this objective by exploiting the \textit{spatial dimension} of
coflows, \ie a coflow typically consists of many flows, via
\textit{sampling}, a highly effective technique used in large-scale
surveys~\cite{samplingOfPopulations}.  In particular, \name pre-schedules
sampled flows, called {\em pilot flows}, of each coflow and uses their measured
size to estimate the coflow size. It then resorts to SCF \addtonreview{(Smallest-Coflow-First)} using the estimated
size.
%job size.

Intuitively, such a sampling scheme avoids all three sources of overhead in
Aalo -- Once the coflow sizes are learned, the coflows are assigned to the
correct queues, which avoids the intrinsic queue-transit and round-robin
effects.
% {Furthermore, directly learning the coflow sizes avoids the
%  need for frequent updates of coflow bytes sent-so-far from local ports.}
Further, a sampling-based design has an important benefit -- it offers much higher
scalability than priority-queue-based learning in Aalo. This is because unlike Aalo, after estimating
the coflow size, \name clients do not need to send periodic updates of bytes
sent-so-far to the centralized coordinator.

%    We analyze this property of \name in
%    \S\ref{sec:scalability} and experimentally demonstrate its scalability in \S\ref{sec:eval}.

% sampling only a small subset of the flows avoids the amplification effect across multiple ports.

\if 0
Conceptually, scheduling pilot flows first before the rest of the flows 
appears to negatively affect CCT in two ways.  First, scheduling pilot flows of a
newly arriving coflow consumes port bandwidth which can delay other
coflows (with already estimated sizes).
%
Second, scheduling pilot flows first may elongate the CCT of the newly arriving
coflow itself whose other flows cannot start until the pilot flows finish.
\if 0
This however is a concern only if the coflow has few flows, \ie one
flow per port, since if a coflow has multiple flows at each port,
sampling a single flow first, \ie serializing the flows, is making the
same progress as other ways of scheduling those flows, as long as the
same bandwidth is allocated to that coflow at that port.  If a coflow
has few flows, \name bypasses the sampling phase, and directly
schedule all its flows at the same priority as other sampled flows.
\fi
%
Our key insight is that
% there will be some overhead associated with any online
% coflow size learning scheme, and the key insight here is that
compared to the multi-queue based approach, the overhead from
sampling-based learning will be much smaller.

Second, we present the complete \name design that addresses four major design issues:
% (1) How to select pilot flows for each newly arriving coflow?
% (2) How to schedule the pilot flows?
(1) How to choose and schedule the pilot flows for each newly arriving coflow?
(2) How to schedule among all the coflows with estimated sizes?
(3) How to schedule flows within a scheduled coflow?
\fi

Developing a complete non-clairvoyant coflow scheduler based on the simple sampling idea raises
three questions:
(1) Why is sampling more efficient than the priority-queue-based coflow size learning? 
(2) Will sampling be effective in the presence of skew of flow sizes?
(3) How to design the complete scheduler architecture?
We systematically address these questions with design rational, theoretical analysis,
system design, prototyping, and extensive evaluation.

\if 0
We evaluated prototype implementation of \name on a 150-node
cluster in Microsoft Azure, and large-scale simulations utilizing a
public MapReduce trace from Facebook by varying the degree of flow size skew.
Our simulation results show that, compared to
prior art Aalo, \name reduces the CCT by 1.78$\times$ (median) and
9.58$\times$ (P90). 
{We also evaluated \name on a testbed by keeping the fraction of the
  time spent by each job in the communication phase the same as given in
  Aalo~\cite{aalo:sigcomm15}.
Our testbed evaluation shows that \name reduces the average job completion time by 18\%
compared to Aalo.
}
\fi

\if 0
In summary, this paper makes the following contributions:
\begin{itemize} %% [noitemsep,topsep=0pt,leftmargin=0.2in]
\item Using a production datacenter trace from Facebook, we show that
  the prior art scheduler Aalo spends substantial amount of time and
  network bandwidth in learning coflow sizes, which negatively
  affects the CCT of coflows.
\item We propose the novel idea of applying sampling in the spatial dimension
of coflows to significantly reduce the overhead of learning coflow sizes online.
% which is needed to approximate the class of SJF-like scheduling algorithms online.
%   The technique can be generalized to other scheduling
%   problems in distributed settings such as cluster job
%   scheduling~\cite{delay:eurosys10}.
\item We present the design and implementation of \name.
\item We extensively evaluate \name via simulations and testbed
  experiments, and show that compared to the prior art, the new design reduces
the average CCT by 1.51$\times$ for the Facebook coflow
trace {and by 1.36$\times$ for a trace with properties similar to a Microsoft production cluster}.
\item The CCT improvement mainly stems from the reduction in the penalty (in
terms of latency and amount of data sent) in determining the right priority queue for
the coflows. \name reduces the median latency and data sent in finding the
right queue for coflows in Aalo by 19.0$\times$ and 20.0$\times$, respectively.
  (\S\ref{sec:sim:probeOverhead}).
\end{itemize}
\fi

In summary, this paper makes the following contributions:
%\begin{itemize} %% [noitemsep,topsep=0pt,leftmargin=0.2in]
\vspace{0.05in}
\noindent
%\item
{\bf (1)} Using a production datacenter trace from Facebook, we show that
  the prior art scheduler Aalo spends substantial amount of time and
  network bandwidth in learning coflow sizes, which negatively
  affects the CCT of coflows.\\
%\item 
{\bf (2)} We propose the novel idea of applying sampling in the spatial dimension
of coflow to significantly reduce the overhead of online learning coflow sizes.\\
% which is needed to approximate the class of SJF-like scheduling algorithms online.
%   The technique can be generalized to other scheduling
%   problems in distributed settings such as cluster job
%   scheduling~\cite{delay:eurosys10}.
%\item 
{\bf (3)} We present theoretical underpinning explaining why
sampling remains effective in the presence of flow size skew.\\
%\item 
{\bf (4)} We present the design and implementation of \name.\\
%\item 
{\bf (5)} We extensively evaluate \name via simulations and testbed
 experiments, and show that compared to the prior art, the new design reduces
the average CCT by 1.51$\times$ for the Facebook coflow
trace {and by 1.36$\times$ for a trace with properties similar to a Microsoft production cluster}.\\
%\item 
{\bf (6)} The CCT improvement mainly stems from reduced coflow size learning overhead.
%  the reduction in the penalty (in
%  terms of latency and amount of data sent) in determining the right priority queue for
%  the coflows.
\name reduces the median latency and data sent in finding the
right queue for coflows in Aalo by 19.0$\times$ and 20.0$\times$, respectively (\S\ref{sec:sim:probeOverhead}).\\
%\end{itemize}
\addtonreview{The rest of the paper is organized as follows. 
\S\ref{sec:back} gives background on the existing studies of coflow scheduling and states the problem we are solving in this paper. 
\S\ref{sec:key} presents the key idea behind our solution and presents qualitative, theoretical, and experimental arguments in its favor. 
\S\ref{sec:design} and \S\ref{sec:impl} discuss design, scalability, and implementation details of \name.
\S\ref{sec:eval-high} summarizes the evaluation results with details presented in \S\ref{sec:sim} (simulation) and \S\ref{sec:eval} (testbed). 
We then discuss related work and conclude.}

==> outline.tex <==
S1: Intro
S2: Background
    -- 2.1: coflow scheduling
    -- 2.2: Aalo design
    -- 2.3: Aalo's limitation: (1) out-of-sync, (2) long delay in determining right queue

S3: Core Ideas
    -- Insight: The key root-cause of the limitations is that Aalo completely missed out the spatial dimension.
    -- 3.1: All-or-none
    -- 3.2: LCoF to reduce average waiting time
    -- 3.3: Per-flow queue thresholds to determine queue faster

S4: Design
    -- 4.1: Architecture (co-ordinator decides the schedule)
    -- 4.2: Scheduling algorithm (main loop for all-or-none, work conservation for rest)
    -- 4.3: Starvation avoidance

S5: Handling cluster dynamics
    -- 5.1: Speeding up coflows with skew, failures and stragglers.
            (We move the coflows from lower to higher priority queues if they have small set of flows pending)
    -- 5.2: Unavailability of data
    -- 5.3: DAGs and multiple waves

S6: Implementation

S7: Testbed

S8: Simulation

S9: Related Work

S10: Conclusion

Appendix: SJF is not optimal. 


==> rate_alloc.tex <==
\vspace{-0.1in}
\subsection{Rate allocation}
\label{sec:design:rate}

Once the scheduling order of the coflows is determined, we need to
determine the rates for the individual flows at each port.
%
First, since we want to quickly finish the pilot flow, at any port that has
pilot flows, \name assigns the \textit{entire} port bandwidth to
the pilot flows.
For the remaining ports, as discussed
in \S\ref{sec:design:starvation}, across multiple queues, \name
assigns weighted shares of the port bandwidth,
%  For assigning rates accross queues we follow a design similar
%  to \cite{varys:sigcomm14}, we share time quantas across the
%  queues.
by assigning them varying numbers of
scheduling intervals according to the weights assigned to each priority queues.

Second, at each scheduling interval, \name assigns rates for the flows
of the coflow in the head of the FIFO queue as follows.
% as in MADD~\cite{varys:sigcomm14},
It assigns equal rates at all the ports containing its flows
as there is no benefit in speeding-up its flows at certain
ports when its CCT depends on the slowest flow.
% and this helps in avoid residual bandwidth.
At each port, we could use max-min fairness to schedule the individual flows of
the coflow (to different receivers), and then assign the rate of the slowest
flow to all the flows in the coflow. Afterwards, the port-allocated bandwidths
are incremented accordingly at the coordinator, which then allocates rates for
the next coflow in the same FIFO queue, and so on. {The psuedocode
for the rate assignment procedure is provided in the supplementary material.}

{\paragraph{Heusristic fast rate allocation.} 
\comment{
For online coflow scheduling it is very important for the coordinator to make
real-time decision in the given synchronization cycle, and therefore, the rate
allocation process should be of low time complexity. 
%the scheduling algorithm should be of low time complexity. 
While previous heuristics such as Smallest-Effective-Bottleneck-First and
Minimum-Allocation-for-Desired-Duration in Varys~\cite{varys:sigcomm14} and
Discretized Coflow-Aware Least-Attained Service in Aalo~\cite{aalo:sigcomm15}
have the advantage of minimizing bandwidth wastage, they slow down the
coordinator and as a result the rate allocation process may fail to finish in a
small synchronization cycle. For fast rate calculation,
%In \name we aim to provide a much simpler heuristics.
in our design, instead of usign max-min fairness to assign rates among
the flows of the head-of-queue coflow,
we use a simple scheme where we assign the \textit{entire}  available bandwidth
corresponding to a priority queue
% (depending on the weight)  
at the sender and receiver ports to one flow of the coflow at the head of the
FIFO queue at a time.  We found that this simple scheme has very marginal
effect on CCTs but makes the rate assignment process considerably faster.
}

%Though the above max-min approach has the advantage of minimizing
%bandwidth wastage, it slows down the coordinator which has
%to iterate over many flows. In our experiments, we used a simple
%scheme where we assign the \textit{entire} bandwidth
%% (depending on the weight)  
%at the sender and receiver ports to one flow of the coflow at the head of the FIFO
%queue at a time.  We found that this simple scheme has very marginal effect on
%CCTs but makes the rate assignment process considerably faster.


%\iftoggle{tons}{
%\commenttons{The following psuedocode function, \textbf{RateAssignment}, shows the
%rate assignment procedure in \name.\\}
%\input algo}{}

% {we assume the sender/receiver ports have the same total bandwidth? - aj: yes}
% Thus we adopted this rate assignment scheme in our experiments.


%In \name, we assign the rate of the slowest flow to all the flows of a
%coflow as intuitively there is no benefit in speeding-up flows at certain ports
%when the CCT depends on the slowest flow.
%\comment{
%At a port, we use max-min
%fairness to schedule the individual flows of a coflow (to different
%receivers).
%}


%   \addaj{However, since \name tries to schedule only one pilot flow of a Coflow
%   at a port, hence bandwidth assigned to a pilot flows is $min(B(s),B(r))$ and
%   they do not share bandwidth with other flows of the parent Coflow at same
%   port.}
%Once the scheduling order of the Coflows is determined, we need
%to determine the rates for the individual flows of a Coflow. One can
%simply assign the \textit{entire} bandwidth 
%% (depending on the weight)  
%at all sender and receiver ports to the Coflow at the head of the
%queue. However, such bandwidth allocation can be wasteful when there
%are uneven numbers of senders and receivers in a Coflow. For a
%Coflow with $s$ sender and $r$ receiver ports, if the bandwidth of
%each port is $B$, the bandwidth assigned to each flow is
%$b = \frac{B}{max(s,r)}$, and the bandwidth utilization (fraction of
%bandwidth used) at each of the sender and receiver ports are
%$\frac{r}{max(s,r)}$ and $\frac{s}{max(s,r)}$,
%respectively, since there are $r$ flows at each sender and $s$
%  flows at each receiver. Thus, when $s \neq r$, either the sender or
%receiver ports will be underutilized. To improve bandwidth
%utilization, \name assigns flow rates depending on the available
%bandwidth as follows.
%
%In \name, we assign the rate of the slowest flow to all the flows of a
%Coflow as there is no benefit in speeding-up flows at certain ports
%when the CCT depends on the slowest flow. At a port, we use max-min
%fairness to schedule the individual flows of a Coflow (to different
%receivers). 


==> rebuttal.tex <==
\abstract
This document contains rebuttal for Paper ID 84.
\vspace{-0.1in}
\section{Rebuttal}
\label{sec:sim}
Text
\vspace{-0.1in}
\subsection{[Simulation] Sensitivity Analysis}
\label{sec:sim:sa}
Text


==> sensitivity.tex <==
\vspace{-0.1in}
\subsection{Sensitivity analysis}
\label{sec:sim:sa}


Compared to Aalo, \name has only two additional paramaters: thinLimit and flow
sampling rate. We already discussed the choice of sampling rate in
\S\ref{sec:sim:pilotflow}.  Below, we evaluate the sensitivity of \name to
thinLimit and other design parameters common to Aalo by varying one parameter
at a time while keeping the rest as the default.

%    Due to space limitation we include the details in the supplementary
%    material of the submission.  In summary, the CCT improvement of \name
%    over Aalo remains largely stable as we vary the thin coflow bypassing limit,
%    start queue threshold, and multiplication factor.}

\begin{figure*}[t]
\label{fig:sim:sa:queues}
\subfigure[Thin coflow bypass threshold]{\label{fig:sim:sa:thinLimit}\includegraphics[width=0.33\linewidth]{figs/sa-TL.eps}}
\subfigure[First queue capacity ($Q_{0}^{\text{hi}}$)]{\label{fig:sim:sa:queues:startQ}\includegraphics[width=0.33\textwidth]{figs/sa-q0.eps}}
\subfigure[Exponent ($E$)]{\label{fig:sim:sa:queues:expo}\includegraphics[width=0.33\textwidth]{figs/sa-qMult.eps}}
\vspace{-0.2in}
	\caption{[Simulation] \name sensitivity analysis. We vary one parameter
of \name keeping rest same as default and compare it with
Aalo.}
\vspace{-0.2in}
\end{figure*}
%\end{figure}

\paragraph{Thin coflow bypassing limit ($T$)} In this experiment, we vary 
thinLimit (T) in \name for bypassing coflows from the probing phase. The result
in Fig.~\ref{fig:sim:sa:thinLimit} shows that the average CCT remains almost
the same as T increases. This is because the average CCT is dominated
by wide and large coflows, which are not affected by thinLimit.
However, the P50 speedup increases till $T = 7$ and
tapers off after $T = 7$.  The reason for the CCT improvement until $T = 7$
is that all flows of thin coflows (with width $\leq 7$) are scheduled
immediately upon arrival which improves their CCT, and the number of
thin coflows is significant. 
%{aj: with our definition 49\% coflows are thin. I have changed the above sentence.}

\paragraph{Start queue threshold ($Q^{hi}_{0}$)}
We next vary the threshold for
the first priority queue from 2 MB to 64 MB.
Fig.~\ref{fig:sim:sa:queues:startQ} shows the average CCT of \name over Aalo.
Overall, \name is not very sensitive to the threshold of first priority queue and the
CCT speedup over Aalo is within 8\% of the default \name (10 MB).
The speedup appears to oscillate with a periodicity of 5x to 10x.
For example, the speedups for 2 MB and 64 MB are close to that
of the default (10 MB), while for 4 MB and 32 MB are lower.
This can be explained by the impact of the first queue threshold
on job segregation; with the default queue threshold growth factor of 10,
every time the first queue threshold changes by close to 10x,
the distribution of jobs across the queues become similar.

\if 0
Fig.~\ref{fig:sim:sa:queues:startQ} shows the average CCT of \name over Aalo.
\name is not very sensitive to the threshold of first priority queue and the
CCT speedup over Aalo is within 8\% of the default \name. For 2 MB, the
performance is similar to the default \name (10 MB) as the threshold
for lower priority queues got doubled up and essentially did not make much
difference in how coflows are being segregated in queues. However, with the
first queue threshold as 4 MB, the way coflows are being segregated, especially
the larger ones, is changing and so we have a slight difference  (8\%)  in
performance as compared to the default \name.  
With the threshold of 8 MB (next to default on the lower side) and 16
MB (next to default on the higher side), it is again similar to the default,
with again slight fluctuation on increasing the threshold further.
\fi

\paragraph{Multiplication factor ($E$)} In this experiment, we vary the queue
threshold growth factor from 2 to 64.  Recall that the queue thresholds are
computed as $Q^{hi}_{q} = Q^{hi}_{q-1} \cdot E$. Thus, as E grows, the number
of queues decreases. As shown in Fig.~\ref{fig:sim:sa:queues:expo}, smaller queue
threshold multiplication factor which leads to more queues performs better
because of fine-grained priority segregation. 

\if 0
\paragraph{Number of priority queues (K)} We next vary the number of priority
queues K.  Fig.~\ref{fig:sim:sa:queues}(b) shows that \name performs poorly
when the number of priority queues is fewer than 8. This can be explained as
follows.
%In this experiment, we keep the start queue threshold and queue threshold
%multiplication factor the same and measure \name's sensitivity to total number
%of priority queues.
With $Q_0^{hi}$ and $E$ unchanged, decreasing the total number of priority
queues by $N$ means that the last  $N+1$ priority queues are collapsed into
one, \ie these large-sized coflows which should have gone into different queues
cannot be efficiently separated.  Meanwhile, small-sized coflows bypass the
priority queues and do not suffer.In the extreme case where the number of
priority queue is reduced to $K = 2$, all bypassing coflows achieve good
speedup (the P50 speedup of all the bypassing coflows is 3.0$\times$ and P10
speedup is 1.0$\times$) and all non-bypassing coflows are having poor speedup
(the P50 speedup of all the non-bypassing coflows is 0.13$\times$ and P90
speedup is 0.89$\times$).  Because in the FB trace, most of the traffic is
concentrated in the few large coflows (the top 0.95\% (3.8\%) largest coflows
form 53\% (95\%) the total traffic), failure to segregate and prioritize large
coflows inflates the average CCT {for \name as compared to the Aalo}
significantly, by 7.7$\times$ (inverse of 0.13) for K=2. 

\paragraph{Weighted bandwidth sharing ($B$)} Recall that to avoid starvation
\name performs weighted bandwidth sharing across different priority queues.  In
this experiment, we vary the ratio of weighted sharing from 2 to 64.  As shown
in Fig.~\ref{fig:sim:sa:queues}(d), with lower values of $B$, \name's
performance deteriorates. This is because of lower values of $B$ result in
increase in share of lower priority queues.
\fi



==> short-sensitivity.tex <==
\vspace{-0.1in}
\subsection{Sensitivity Analysis}
\label{sec:sim:sa}
Next, we evaluate the sensitivity of \name to different design
parameters.
\vspace{-0.05in}
\paragraph{Thin coflow bypassing limit ($T$)}
In this experiment, we vary the thinLimit (T) in \name for bypassing coflows from
the probing phase. The results in Fig.~\ref{fig:sim:sa:thinLimit} shows that the
average CCT remains almost the same as T increases.  However, the P50 speedup
increases till $T = 7$, and tapers off after $T = 7$.
The key reason for the CCT improvement until $T = 7$ is that
all flows of the thin coflows (with width $\leq 7$) are scheduled immediately
upon arrival which improves their CCT (\S\ref{sec:design:additional}), and the majority of
the coflows are thin.

\paragraph{Start queue threshold ($Q^{hi}_{0}$)} We next vary the threshold for
the first priority queue from 2 MB to 64 MB. Fig.~\ref{fig:sim:sa:queues:startQ}
shows as the average CCT. \name is not very sensitive to the threshold of first
priority queue and fluctuation from default is at most 8\%. For 2 MB the performance
is similar to default \name as the threshold for lower priority queues got
doubled up and essentially did not make much difference in how coflows are
being seggregated in queues. However, with the first queue threshold as 4 MB,
the way coflows are being seggregated, especially the larger one's, is changing
and so we have slight (8\%) difference in performance as compared to default.
However, with the threshold being 8 MB and 16 MB it is again similar to the
default with again slight fluctuation on increasing the threshold further.  

\paragraph{Multiplication factor ($E$)} In this experiment, we vary the queue
threshold growth factor from 2 to 64.  Recall that the queue thresholds are
computed as $Q^{hi}_{q} = Q^{hi}_{q-1} \cdot E$. Thus, as E grows, the number
of queues decreases. As shown in Fig.~\ref{fig:sim:sa:queues:expo}, smaller queue
threshold multiplication factor which leads to more queues performs better
because of fine-grained priority segregation. 


==> simulation.tex <==
\begin{table*}[htbp]
	\centering
\label{table:sim:sa:probeSelection}
\caption{Performance improvement over Aalo for varying pilot
          flow selection schemes.
}
\vspace{-0.2in}
{\small	
	\begin{tabular}{ccccccccccc}
		\\ \Xhline{3\arrayrulewidth}
	&	\multicolumn{1}{c|}{Constant} & \multicolumn{5}{c|}{Proportional to number of senders}     & \multicolumn{2}{c}{Proportional to number of flows} \\ 
	   & \multicolumn{1}{c|}{2} & 5\% & 10\% & 20\%& 50\%  & \multicolumn{1}{c|}{100\%} & 1\%      & 10\%                 \\  \Xhline{3\arrayrulewidth}
			    	Avg. error &13.21\%&6.14\%&5.42\%&4.94\%&5.53\%&4.25\%&4.15\%&2.90\%                                    \\
				Avg. CCT  &1.27$\times$&1.51$\times$&1.45$\times$&1.50$\times$&1.50$\times$&1.50$\times$& 1.43$\times$&0.49$\times$ \\ 
				P50 speedup &1.75$\times$&1.78$\times$&1.76$\times$&1.71$\times$&1.52$\times$&1.40$\times$& 1.33$\times$&0.69$\times$  \\
				P90 speedup &9.00$\times$&9.58$\times$&9.00$\times$&9.15$\times$&8.33$\times$&8.45$\times$& 8.23$\times$&8.23$\times$  \\

\hline
	\end{tabular}
}
\vspace{-0.2in}
\end{table*}
\section{Evaluation Highlights}
\label{sec:eval-high}

We evaluated \name using a 150-node and a 900-node testbed cluster in Azure and
using large scale simulations by utilizing a publicly available
{Hive/MapReduce} trace collected from a 3000-machine, 150-rack Facebook
production cluster~\cite{fbtrace:web} and multiple derived traces with 
varying degrees of flow size skew to measure \name's robustness to skew.

%\addaj{Skew in flow size(data) of a coflow is the property which can most
%influence \name's performance. Hence, along with subsets of the FB-trace,
%which have high data-skew across flows of a coflow we also evaluated \name on
%a trace with data skew similar to what is observed in a production cluster
%from Microsoft(\S\ref{sec:sim:skew}).}
%\begin{itemize}
%\item {\bf Facebook (FB) trace}:
{\bf Facebook (FB) trace}:
{The trace contains 150 ports and 526 ($> 7 \times 10^{5}$ flows) coflows, that
are extracted from Hive/MapReduce jobs from a Facebook production cluster.}
{Each coflow consists of pair-wise flows between
a set of senders and a set of receivers.
}
\if 0
    {The trace only contains information about
the total data received at each reducer and so the total data of a reducer is equally
divided among all the incoming flows to a reducer.}
\fi 
%\end{itemize}

Due to the lack of other publicly available coflow trace\footnote{A challenge that has
also been faced by previous work on coflow scheduling such as~\cite{sunflow:conext16,
zhang:sigcomm15, aalo:sigcomm15} and \cite{graviton:hotcloud16}.},
we derived three additional { classes} of traces using
%\editaj{from}{using} 
the original Facebook trace in order to more thoroughly evaluate 
\name under varying coflow size skew:\\
%\begin{itemize}
%\item 
{\bf Low-skew-filtered}: Starting with the FB trace,
we filtered out coflows that have
skew (\emph{max flow length}/\emph{min flow length}) less than a
constant $k$. We generated five traces in this class with $k =
1,2,3,4,5$. {The filtered traces have 142, 100, 65, 51 and 43 coflows, respectively.}\\
%\item 
{\bf Mantri-like}: Starting with the FB trace, we adjusted the sizes of
the flows sent by the mappers,
keeping the total reducer data the same as given in the original trace, 
to match the skew of a large {Microsoft} production cluster trace as
described in Mantri~\cite{mantri:OSDI2010}.
{In particular, the sizes are adjusted so that
the coefficients of variation across mapper data are0
about 0.34 in the $50^{th}$ percentile case and 3.1 in the $90^{th}$ percentile case.}
{This trace has the same numbers of coflows and ports as the FB trace.}\\
%\item 
{\bf  Wide-coflows-only}: We filtered out all the coflows in the FB trace
with the total number of flows $\leq 7$, the default thin coflow bypass
threshold (thinLimit) in \name.  {The filtered trace has 269 coflows spreading
over 150 ports.}
%\end{itemize}

% \addtonreview{Along with the testing effect of skew the above traces help us to capture the real world cluster behaviour, as they represent properties of two different Industrial clusters.}
The primary performance metrics used in the evaluation are 
CCT or CCT speedup,
defined as the ratio of a CCT under other
baseline algorithms and under \name, piloting overhead, and coflow size estimation
accuracy.

The highlights of our evaluation results are:
%\begin{itemize}
  %  \editaj{\name significantly reduces the overall CCT over the prior art
  %  Aalo, by 1.78$\times$ in the median case (P90 = 9.58$\times$).}
%\item 
{\bf (1)} \name significantly improves the CCTs. In simulation using the FB trace, the
average CCT is improved by 1.51$\times$ over the prior art, Aalo. Individual
CCT speedups are 1.78$\times$ in the median case (P90 = 9.58$\times$).  For
the Mantri-like trace, the average CCT is improved by 1.36$\times$ and 
individual CCT speedups are 1.75$\times$ in the median case (P90 = 12.0$\times$).\\
%\item 
{\bf (2)} The CCT improvement mainly stems from the reduction in the learning
overhead (in terms of latency and amount of data sent) in determining the right
queue for the coflows. Compared to Aalo, median reduction in the
absolute latency 
%\comment{absolte or reative? aj: ratio of time taken by aalo to time taken by
%\name}
in finding the right queue for coflows in \name is 19.0$\times$, and
% median reduction
in absolute amount of data sent is 20.0$\times$ (\S\ref{sec:sim:probeOverhead}).\\
%\item
{\bf (3)} \name improvements are consistent when varying the skew among the
flow sizes in a coflow (\S\ref{sec:sim:skew}).\\
%\item
{\bf (4)} \name is robust to parameter variation (\S\ref{sec:sim:sa}).\\
%{\bf (4)} \name improvements are consistent when varying its parameters (\S\ref{sec:sim:sa}).\\
%\item
%{\bf (5)} Compared to Aalo the \name coordinator is highly scalable (\S\ref{sec:eval:scale}).\\
{\bf (5)} The \name coordinator is much more scalable than that of Aalo (\S\ref{sec:eval:scale}).\\
%\end{itemize}

\vspace{-0.2in}
\section{Simulation}
\label{sec:sim}
%\vspace{-0.05in}
We present detailed simulation results in this section, and the testbed
evaluation of our prototype in \S\ref{sec:eval}.

%\vspace{-0.05in}
\paragraph{Experimental setup:}
\label{subsec:setup}
% In replaying the trace, we maintain the same flow lengths and flow ports. 
Our simulated cluster uses the same number of nodes (sending and
receiving network ports) as in the trace.
As in~\cite{aalo:sigcomm15}, we assume full bisection
bandwidth is available, and congestion can happen only at network
ports.

The \textit{default parameters} for Aalo and \name in the experiments are:
starting queue threshold ($Q^{hi}_0$) is 10MB, exponential threshold growth
factor ($E$) is 10, number of queues ($K$) is set to 10, the weights assigned
to individual priority queues decrease exponentially by a factor of 10, and 
%Aalo the new schedule calculation interval $\delta$ is set to 8ms as suggested
the new schedule calculation interval $\delta$ is set to 8ms for the 150-node cluster {\footnote{8ms is the time to send 1MB of data.}}, the default
suggested in its publicly available simulator~\cite{aalo:sigcomm15}. In \name,
a new schedule is calculated on demand,
upon arrival of a new coflow,
  completion of a coflow, or completion of all pilot flows of a coflow.

Finally, in \name
the threshold for thinLimit (T) is set to 7, the number of pilot flows
assigned to wide coflows are $max(1, 0.05 \cdot S$), where $S$ is the number of
senders, and the default inter-coflow scheduling policy in \name is
{Least length-weighted total-port contention}.

%\vspace{-0.15in}
\subsection{Pilot flow selection policies}
\label{sec:sim:pilotflow}

We start by evaluating the impact of different policies in choosing
the pilot flows for a coflow in \name.
Table~\ref{table:sim:sa:probeSelection} summarizes the improvement in
average CCT of \name over Aalo and average error in size estimation
normalized to the actual coflow size, when varying the pilot flow
selection policy while keeping other parameters as the default in \name, using the FB trace.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%							%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	Below is minipage fitted table and figure	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%							%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if 0

\begin{figure*}
%\begin{minipage}{\textwidth}
\begin{minipage}{0.3\textwidth}
%\begin{figure}[tp]
%\centering
\includegraphics[width=0.9\linewidth]{figs/EstAcc-scatter.pdf} %done
\captionof{figure}{\name coflow size learning accuracy. Coflows that did not go through
the piloting phase (48\%) are not shown.
\vspace{-0.1in}
%\updated{05/25/2018}
}
\label{fig:sim:estimationAccuracy}
%   the probing phase (40\%)}
% \label{fig:sim:probingEffectiveness}
%\end{figure}

\end{minipage}
\hfill
\begin{minipage}{0.68\textwidth}
%\begin{table*}[tp]
	\centering
\captionof{table}{Performance improvement over Aalo for varying pilot
          flow selection schemes.
}
	\label{table:sim:sa:probeSelection}
{\small	
	\begin{tabular}{ccccccccccc}
		\\ \Xhline{3\arrayrulewidth}
	&	\multicolumn{1}{c|}{Constant} & \multicolumn{5}{c|}{Proportional to num(Senders)}     & \multicolumn{2}{c}{Proportional to number of flows} \\ 
	   & \multicolumn{1}{c|}{2} & 5\% & 10\% & 20\%& 50\%  & \multicolumn{1}{c|}{100\%} & 1\%      & 10\%                 \\  \Xhline{3\arrayrulewidth}
			    	Avg. error &13.21\%&6.14\%&5.42\%&4.94\%&5.53\%&4.25\%&4.15\%&2.90\%                                    \\
				Avg. CCT  &1.27$\times$&1.51$\times$&1.45$\times$&1.50$\times$&1.50$\times$&1.50$\times$& 1.43$\times$&0.49$\times$ \\ 
				P50 speedup &1.75$\times$&1.78$\times$&1.76$\times$&1.71$\times$&1.52$\times$&1.40$\times$& 1.33$\times$&0.69$\times$  \\
				P90 speedup &9.00$\times$&9.58$\times$&9.00$\times$&9.15$\times$&8.33$\times$&8.45$\times$& 8.23$\times$&8.23$\times$  \\

\hline
	\end{tabular}
}
%\vspace{-0.1in}
%\end{table*}
\end{minipage}
%\end{minipage*}
\end{figure*}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%							%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	Above is minipage fitted table and figure	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%							%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% The error rate is calculated as $$
%% \frac{|\text{Estimated Job Size - Actual Job Size}|}{\text{Actual Job
%%     Size}} $$

Unsurprisingly, the estimation accuracy increases when increasing the
number of pilot flows across the three selection schemes: constant,
fraction of senders, and fraction of total flows. However, as the
number of pilot flows increases (over the range of parameter
choices), the CCT speedup (P50 and P90 {of individual coflow CCT
  speedups}) decreases. This is because the benefit from size
estimation accuracy improvement from using additional pilot flows does
not offset the added overhead from completing the additional pilot
flows and the delay they incur to other coflows.

%  Also, for thin coflows, better estimation which comes at the cost of
%  elongated probing time does not help in reducing post probing time
%  proportionally.

%While increasing the number of pilot flows proportional to the number of
%senders, the change in average CCT is not very considrable as average CCT is
%dominated by the larger coflows.
%
We find sampling 5\% of the number of senders per coflow strikes a
good trade-off between piloting overhead and size estimation accuracy
leading to the best CCT reduction. We thus set it
($0.05\cdot S$) as the default pilot flow selection policy.
%% to estimate size and hence to achieve optimal
%% ordering increases, this is the reason of poor average
%% improvements. Poor average CCT improvement for constant number of
%% pilot flows is due to large error in size estimation.

%\vspace{-0.2in}
\subsection{Piloting overhead and accuracy}
\label{sec:sim:probeOverhead}
\begin{figure}[!htbp]
\centering
\vspace{-0.22in}
\includegraphics[width=0.9\linewidth, natwidth=610,natheight=642]{figs/EstAcc-scatter.pdf} %done
\vspace{-0.15in}
\caption{\name coflow size learning accuracy. Coflows that did not go through
the piloting phase (48\%) are not shown.
%\updated{05/25/2018}
}
\vspace{-0.1in}
\label{fig:sim:estimationAccuracy}
%   the probing phase (40\%)}
% \label{fig:sim:probingEffectiveness}
\end{figure}

%% \TODOAJbyRG{Akshay -- this figure is not very useful. Can you please
%%   plot a scatter-plot. X-axis is actual size, Y-axis is estimated
%%   size? Or, show the ratio across 4 bins. Also, what's the use of this
%%   figure? The difference in estimation/actual is because of the skew?
%%   An interesting graph would be sensitivity to number of pilot flows.}
%% \\{We will add a table with average error in estimation with 
%% different piloting schemes. Sure the difference might be due to skew 
%% and it is \name's job to estimate correct size. This figure show's that 
%% how well it is doing that. Skew is a property of real world trace and
%% cannot be eliminated}

Next, using the default pilot selection policy,
we evaluate \name's effectiveness in estimating coflow sizes by sampling
pilot flows. Fig.~\ref{fig:sim:estimationAccuracy} shows a scatter plot of the
actual coflow size vs. estimated size from running \name under the default
settings.  We observe that \name coflow's size estimation is highly accurate
except for a few outliers. Overall, the average and standard deviation of
%relative estimation error are 0.06 and 0.15, respectively, and for the top 99\%
%(95\%) coflows (in terms of accuracy), the average and standard deviation of
%relative error are only 0.05 (0.03) and 0.12 (0.07).
relative estimation error are 0.06 and 0.15, respectively, and for the top 99\%
and 95\% coflows (in terms of estimation accuracy), the average (standard
deviation) of relative error are only 0.05 (0.12) and 0.03 (0.07) respectively.
%\comment{numbers worng?? aj: No. I think it was written in confusing way. I
%have changed it please read it.}
Interestingly, a few
coflows experience large estimation errors, and we found they all have very
high skew in their flow lengths; the mean standard deviation in flow lengths,
normalized by the average length, of the bottom 1\% (in terms of accuracy)
ranges between 4.6 and 6.8.

%In this section we evaluate effectiveness of the process of estimating coflow
%size by probing, to do so we perform two different experiments, results of
%which are shown in Fig.~\ref{fig:sim:probingEffectiveness}. Fig.
%~\ref{fig:sim:estimationAccuracy} demonstrates the accuracy of the estimation.
%Size of around 40\% of the coflows, which were probed, is estimated precisely
%and for another \~45\% it is estimated within 20\% error margin.

Fig.~\ref{fig:sim:learningCost} shows the cost of estimating the correct queue
for each coflow in \name and Aalo, measured as the time in learning the coflow
size as a fraction of the coflow's CCT in \name and Aalo. We see that under
\name, about 63\% of the coflows spent less than 1\% of their CCT in the
learning phase, while under Aalo, 63\% coflows reached the correct priority
queue after spending up to 22\% of their CCT moving across other queues.
{Compared to Aalo, \name in the median case sends 20$\times$ less data in
determining the right queue and reduces the latency in determining the
right queue by 19$\times$.}

%(\TODOAJbyRG{why? reasons? Also, why compare 60\$ an 80\%. Keep them the same}).

%Fig. ~\ref{fig:sim:learningCost} is to measure cost of estimation. The plots are CDF
%of fraction of total time spent in learning correct size of the coflow. For
%\name time spent in learning is the time spent in probing phase and for AALO it
%is the time used to reach the end queue \ of coflow. More than 80\% of the
%coflows which, went through probing took less than 1\% of their CCT in learning
%phase. In contrast for AALO, more than 60\% of the coflows took more than 50\%
%time in learning learning phase.

\subsection{Inter-coflow scheduling policies}
\label{sec:sim:intercoflows}


\name differs from Aalo in two ways: online size estimation and inter-flow scheduling policy.
Here, we evaluate the effectiveness of the {four} inter-coflow
scheduling policies of \name discussed in \S\ref{sec:design:intercoflow},
keeping the remaining parameters as the default. Such evaluation allows us to
decouple the contribution of sampling-based learning from the effect of
scheduling policy difference.


Table~\ref{table:inter-coflow} shows the CCT improvement of \name
under the four inter-flow scheduling policies over
Aalo. We make the following observations.
%% We can define diverse metrics of how the scheduler plugs coflows into
%% different priority queues based on information such as estimated job
%% size and arrangement of coflows accross ports(space). In table
%% \ref{table:inter-coflow} we list median and P90 speedUps and
%% improvement in average CCT as compared to Aalo for five different
%% metrics we explored other than the final design of \name. For this
%% experiment we kept all the other design components exactly same as in
%% \name. We make following observations:

First,
%  \editaj{the purely sized-based policy, {\bf Smallest job first (A)},
%  already significantly outperforms Aalo, reducing the average CCT by
%  1.40$\times$, from accurate and efficient estimation of coflow sizes. }
\name with the purely sized-based policy, {\bf Smallest job first
(A)}, which uses the same inter-queue and intra-queue scheduling policy as Aalo and
  only differs from Aalo in coflow size estimation,
  % (sampling vs moving coflows across queues),
  reduces the average CCT (P50) of Aalo by 1.40$\times$ (1.48$\times$).

%  In contrast,
%  the default \name which uses the total-port contention policy (D)
%  reduces the average CCT (P50) of Aalo by 1.51x (1.78x).
%  These results indicate that the primary improvement in \name comes from its
%  sampling-based coflow size estimation scheme.}


In contrast, the default \name uses
{\bf Least length-weighted total-port contention (D)}, which uses the sum of
size-weighted port contention to assign coflows to priority queues, 
and slightly outperforms the size-based policy A;
it reduces the average CCT (P50) of Aalo by 1.51$\times$ (1.78$\times$).
This is because it captures the
diversity of contention at different ports, which happens often in real
distributed settings, and at the same time accounts for the coflow size by
using length-weighted sum of the port-wise contention. 
The above results for policy A and policy D
indicate that the primary improvement in \name comes from its
sampling-based coflow size estimation scheme.


{\bf Shortest remaining time first (B)}
performs similarly as smallest job first. {This is because the preemptive
nature of SRTF will kick in only on arrival of new coflows}.
%  {As the pre-emptive
%  nature of the SRTF kicks in only on arrival of new entities in the system, as
%  no existing job can have shortest-remaining-time than then one which is
%  currently scheduled.\\}
%  {why isn't SRTF trigerred at every scheduling cycle???}
%  {There is no concept of scheduling cycle in \name as lengths are
%  estimated on arrival only and contention will change only on arrival or
%  completion of flows. So scheduling order changes only on arrival of coflows and
%  completion of flows}\\
%  {Also, even if there will be scheduling at every cycle -- I am saying
%  that pre-emptive nature of SRTF will only kick in on arrival of new job as the
%  one which is currently scheduled(i.e. job with SRT) will remain to be one with
%  SRT among the existing jobs. -- This is will happen in any SRTF case. I have
%  modified the earlier sentence a bit to make this more explicit. Let me know if
%  that is good.}\\
Also, although SRTF is advantageous for small coflows, since \name already
schedules thin coflows at high priority, many thin and thus small coflows are
anyways being scheduled at high priority under both policies A and B, and
as a result they perform similarly.

%First, {\bf Shortest remaining size first (B)} actually performs worse
%than {\bf Smallest job first (A)}. This is because this policy will move
%the coflows that start in lower priorities (after size estimation) to
%high priority queues gradually, and since coflows within a queue are
%processed in the FIFO order, they will be waiting for a long time in
%each queue (worse than staying in the original low priority queue).
%However, the CCT of smaller coflows will improve as they are now not
%being blocked by larger coflows priority queues.

Next, {\bf Least global contention first (C)} performs poorly. This is
because global contention for a coflow is defined as the unique number of
other coflows that share ports, and as a result such a policy
completely ignores the size (length) of the coflows.

\iftoggle{tons}{
{%\color{red}	%	closing bracket on line 455 
Finally, {\bf Least length-weighted max-port contention first (E)} and {\bf
Least max length-weighted global contention first (F)} perform better than the
above size-based or contention-only based policies for some coflows, by
incorporating the flow length factor.  However, these two policies sort coflows
based on either an extreme notion (E) or a coarse notion (F) of contentions faced by
coflows at their ports. As a result,
%  the CoFlows that have even one very contentious port are being penalised
%  very heavily.
wider coflows, which tend to have high contention at at-least one of their ports,
are being scheduled with lower priority. This results in 
higher average CCT than {\bf Least length-weighted total-port contention (D)}.
}}{}


\if 0
Fourth, {\bf Least length-weighted contention first (D)} and {\bf Least max
length-weighted port contention first (E)} perform better than the above
size-based or contention-only based policies for some coflows, by incorporating
the flow length factor.  However, these two policies sort coflows based on
coarse notion (D) or extreme notion (E) of contentions 
faced by coflows at their ports. As a result,
%  the coflows that
% have even one very contentious port are being penalised very heavily.
wider coflows which tend to have high contention at at least one of
their ports are being scheduled with lower priority. This results in
poor average CCT.
\fi


\begin{table}[tp]
  \centering
%\vspace{-0.1in}
  \caption{CCT speedup in \name under different inter-coflow scheduling
    policies (\S\ref{sec:design:intercoflow}) over Aalo.}
%\vspace{-0.1in}
  \label{table:inter-coflow}
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccc}
      \Xhline{3\arrayrulewidth}
	    Priority estimation metric & P50 & P90  & Avg. CCT \\ 
      \Xhline{3\arrayrulewidth}
      Estimated size (A)         &1.48$\times$ &  8.27$\times$ &1.40$\times$ \\
      
      Remaining size (B)   &1.54$\times$ & 8.34$\times$ & 1.37$\times$ \\ 
      
      Least global contention first (C) &0.75$\times$ & 8.26$\times$& 0.13$\times$ \\
      
	Length-weighted total-port     & 1.78$\times$   & 9.58$\times$ &1.51$\times$ \\
contention (D) (\name) & & & \\
%	(\name) &&& \\
%\iftoggle{tons}{	% If removing this section you need to make some changes in the e$\times$planation part of these results.And also may be regarding the number of policies tried.
%{\color{red}	%	closing bracket on line 482
      
      Least length-weighted max-port     & 1.43$\times$ & 9.00$\times$& 1.13$\times$   \\
contention first (E) & & & \\
	
	Length-weighted global   & 1.68$\times$& 10.25$\times$ & 1.22$\times$\\
contention first (F) & & & \\
	%}}{}
      \hline
%\vspace{-0.2in}
  \end{tabular}}
\vspace{-0.1in}
\end{table}


%   {Our evaluation result in table ~\ref{table:inter-coflow} shows that
%   the best improvements in individual CCT as well as average CCT is acheived by
%   algorithm $F$. Our insight says that the reason behind $F$ outperforming other
%   desing options is that by taking sum of contention $\times$ length at each
%   port, it is affectively accounting for both time (proportional to length) a
%   coflow will occupy the port as well as the number of other coflows it will
%   affect. We choose $F$ to be default policy for \name's final design.}

\vspace{-0.1in}
\subsection{Average CCT improvement} 
\label{sec:sim:cct}

%\begin{figure}[t] 
%\centering
%%\minipage{0.32\textwidth}
%\vspace{-0.2in}
%% \subfigure[Mix of thin and wide coflows] {
%\includegraphics[width=0.9\linewidth]{figs/PerformanceCompare.pdf}      % done
%%  \label{fig:sim:cctOthers:all}
%\\
%\vspace{-0.1in}
%%\endminipage
%(a) Using original FB trace.
%\\
%%\minipage{0.32\textwidth}
%\includegraphics[width=0.9\linewidth]{figs/PerformanceCompareOnlyWide.pdf}      % done
%%\label{fig:sim:cctOthers:onlyWide}
%\\
%\vspace{-0.1in}
%(b) Using Wide-coflows-only trace.
%\vspace{0.1in}
%\caption{CCT Speedup of \name over other scheduling policies.
%%  On full trace \name achieves median(P90) speedup of 3.0$\times$(77.96
%%  $\times$) and 3.16 $\times$ for average CCT over simple FIFO based
%%  policy. \updated {05/25/2018}
%%  % The Y-axis denotes the improvement in speedups and average cct.
%} 
%%\endminipage
%\label{fig:sim:cctOthers}
%\vspace{-0.1in} 
%\end{figure}

%\minipage{0.25\textwidth}
%\endminipage

\begin{figure} 
\centering
\subfigure[\vspace{-0.2in}Using original FB trace.]
{
%\includegraphics[width=0.24\linewidth]{figs/PerformanceCompare.pdf}
\includegraphics[width=0.48\linewidth, natwidth=610,natheight=642]{figs/PerformanceCompare-testFig7.pdf}% done
\hspace{-0.15in}
\label{fig:sim:cctOthers:fb}
}
\subfigure[\vspace{-0.2in}Using Wide-coflows-only trace.]
{
%\includegraphics[width=0.24\linewidth]{figs/PerformanceCompareOnlyWide.pdf}	% done
\includegraphics[width=0.48\linewidth, natwidth=610,natheight=642]{figs/PerformanceCompare-testFig7-WideOnly.pdf}
\hspace{-0.15in}
\label{fig:sim:cctOthers:onlyWide}
}
\caption{\addtonreview{ CCT speedup using \name compared to using other coflow schedulers on
  different traces.}
  %In Fig.~\ref{fig:sim:cctOthers:skew:lowSkewFilter},
  %%%%%%% shows improvements of \name over Aalo only
%the x-axis denotes the minimum skew in 
%the 5 Low-skew-filtered traces.
%   \addaj{Y-axis denotes speedup i.e. ratio of CCTs}
}
\vspace{-0.2in}
\label{fig:sim:cctOthers}
\end{figure}

We now compare the CCT speedups of \name against 5
well-known coflow scheduling policies: (1) Aalo, (2) Aalo-Oracle,
which is an oracle version of Aalo where the scheduler knows the final
queue of a coflow upon its arrival time and directly starts the
coflow from that queue, (3) SEBF in Varys~\cite{varys:sigcomm14} which
assumes the knowledge of coflow sizes apriori and uses the Shortest
Effective Bottleneck First policy, where the coflow whose slowest flow
will finish first is scheduled first.  (4) FIFO, which is a single
queue FIFO based coflow scheduler, and (5) FAIR, which uses per-flow
fair sharing.
We do not include Saath~\cite{jajooSaath} in the
comparison as it does not provide the same liveliness guarantees as
\name which as discussed in \S\ref{sec:design:starvation}
can obscure the comparison result.
\if 0
%\addaj{and it's all-or-none design inherently leaverages benefits of
%impractical assumption that all the flows of a coflow will be ready at the
%same time.}\\\questionaj{Should we altogether avoid talking about Saath?}.
\fi
All experiments use the default parameters discussed in the
setup, including $K, E, S$, unless otherwise stated.  The results are
shown in Fig.~\ref{fig:sim:cctOthers:fb}. We make the following
observations.

%  \questionaj{I am not sure if we should add the comparison of policy A part here
%  too. Or should be change the next paragraph in anyway.}

  First,
%  to isolate any improvement due to improved scheduling policy
%  from fast size estimation,
we compare CCT under \name against under
Aalo-Oracle, where Aalo-Oracle starts all coflows at the correct priority queues
(\ie no learning overhead). \name improves the average CCT by
%1.18$\times$, and P50 (P90) CCT by 1.40$\times$ (55.00$\times$),
1.18$\times$ and P50 CCT by 1.40$\times$,
respectively.
%  average CCT.
%  {Chengze : (1)
%    Thin limit increase a little bit performance. (2) We are using
%    spatial/contention-based inter-coflow scheduling algo, which
%    outperforms Aalo's SJF. In fact, the estimated SJF in \name is worse
%    than aalo(oracle) by 4\% (shown in table 3).}
Since Aalo-Oracle pays no overhead for coflow size estimation,
its worse performance suggests that using length-weighted total-port
contention in assigning coflows to the priority queues in \name
outperforms Aalo's size-based, contention-oblivious policy in assigning
coflows to the queues.


Second, \name improves the average CCT over Aalo by 1.51$\times$
%(median) and P50 (P90) by 1.78 (9.58$\times$). The significant {\em additional}
(median) and P50 by 1.78. The significant {\em additional}
improvement on top of the gain over Aalo-Oracle comes from fast and
accurate estimation of the right queues for the coflows
(Fig.~\ref{fig:sim:learningCost}).

Third, \name, which requires no coflow size knowledge a priori,
achieves comparable performance as SEBF~\cite{varys:sigcomm14}; it
reduces the average CCT by 1.16$\times$. Again this is because its
total-port contention policy outperforms the contention-oblivious SEBF.

\addtonreview{
Fourth, we compare \name against  Saath \cite{jajooSaath} and Graviton \cite{graviton:hotcloud16}. \name improves over Saath \cite{jajooSaath} and Graviton \cite{graviton:hotcloud16} because of its better and accurate learning. We note that Saath and Graviton like Aalo follow the priority queue based estimation technique. However, Graviton does a better job in sorting the coflows in their assigned queues. Hence, the speedup of Philae over Graviton is slightly lower when compared to Aalo. Average CCT speedup = 1.36$\times$ and 1.31$\times$ for the full trace and wide-coflows-only trace, respectively. Similarly, the speedup of Philae over Saath is lower because of the advanced scheduling policies in Saath like All-or-none. Average CCT speedup = 1.13$\times$ and 1.09$\times$ for the full trace and wide-coflows-only trace, respectively. However, the better performance of Saath and Graviton are not due to their learning technique, because they both use the priority queue based learning techniques similar to that in Aalo to learn coflow sizes. Rather, the gains are due to the more complex versions of the scheduling and coflow sorting techniques than those used in Aalo. Further, in practice Saath and Graviton face the same scalability issues as Aalo (because they have similar global coordinator architecture as they have similar learning techniques). For example, in a 150 port testbed experiment, we observed that Saath uses CPU 3.96$\times$ (3.24$\times$) more than Philae in P50 (P90) case. Similarly, Aalo's CPU usage is also much higher than \name, which is about 3.40x more than \name. Since, in this paper our goal is to evaluate the new sampling-based coflow size estimation technique so we only use Aalo for detailed analysis.}

%  median speedup of 0.9$times$. Additionally, compared to SEBF, \name
%  improves the average CCT improved by 10\%. 

%The key observation is that \name improves the CCT over Aalo by 1.44$\times$
%(median) and 6.21$\times$ (P90). Interestingly, \name achieves median speedup
%of 1 and average CCT improved by 5\% when compared to SEBF in Varys
%~\cite{varys:sigcomm14} even if SEBF runsoffline and assumes the coflow
%sizes are known {\em apriori}, whereas \name runs online without {\em apriori}
%knowledge of coflow sizes.

Finally, \name significantly outperforms the single-queue FIFO-based
coflow scheduler, with a median (P90) CCT speedup of 3.00
%\end
(77.96)$\times$ and average CCT speedup of 3.16$\times$, and the
un-coordinated flow-level fair-share scheduler, with a median (P90) CCT
speedup of 70.82$\times$ (1947.12$\times$) and average CCT speedup of
5.66$\times$.

\if 0
Next, we compare \name against a FIFO-based coflow scheduler under which
coflows are scheduled at individual ports, without any global coordination, in
the order of their arrival time. In this scheme, there are no multiple priority
queues. Lack of coordination, coupled with lack of priority queues, severely
hampers the CCT. \name achieves a median(P90) CCT speedup of 3.0
(77.96)$\times$ and improves the average CCT by 3.16$\times$ over the
FIFO-based scheduler.

%We also compare \name against a FIFO-based coflow scheduler under which coflows
%are scheduled at individual ports, without any global coordination, in the
%order of their arrival time. In the FIFO, there are no queues. Lack of coordination,
%coupled with lack of priority queues severely hampers the CCT in the FIFO. 
%\name achieves a median speedup of 2.25 $\times$ and average CCT
%improves by 187 \% $\times$ against the FIFO based scheduler. 

Finally, we compare \name against an un-coordinated flow level scheduler, where
there are no queues, and all the flows are scheduled upon arrival as per TCP.
Again, lack of coordination, coupled with lack of priority queues and no notion
of coflows, severely hampers the CCT, and \name achieves median(P90) CCT
speedup of 70.82$\times$ (1947$\times$) and average CCT improvement of
5.66$\times$.
% {Can you add another result where you run Aalo but the coflow
%   sizes are already known, and coflows are already placed in the right
%   queue. This shows how close we get to the best case.}
% {Done. However, this is not the best case. As this still ignores the
% spatial dimension. I think Varys is the best case.}
\fi

\if 0
In summary, our results above show that \name is far more effective in
reducing coflow completion time than existing non-clairvoyant coflow schedulers. Further,
it achieves similar performance as SEBF which
assumes prior knowledge of coflow sizes.
\fi

% , and achieves high speedups compared to other un-coordinated scheduler.


To gain insight into how different coflows are affected by \name over
Aalo, we group the coflows in the trace into four bins defined in
Table \ref{table:sim:bin}, and show in Fig.~\ref{figs:speedup:bin} the
CCT speedups for each bin. We see that
\name { improves CCT for all coflows in bin 1 and 3 and for large fraction in bin-4. Most of the underperforming coflows fall in bin-2}. Coflows in bin-2
have width $>$ 7 and size $<$ 100MB, \ie the flows are short but
wide. Because the width exceeds the thinLimit, \name
schedules the pilot flows to estimate the coflow size first
(\S\ref{sec:design}). Thus, although the remaining flows are short, they get delayed
until the completion of the pilot flows, which results in CCT
increase.
%\addaj{We also observed that more than two-third of the coflows which have CCT
%speedup $< 0.5 (P15)$ are wide with $< 2MB$ data per flow. Compared to
%Aalo, \name is not performing well for wide coflows with small flow
%lengths, as most of the short-flow coflows will quickly finish in high
%priority queues in Aalo, whereas in \name they endure the delay from size
%estimation.}


Finally, since thin coflows benefit from \name's scheme of bypassing probing
for thin coflows, we also compare \name with other schemes using the Wide-coflows-only trace which
consists of all coflows wider than {the default thinLimit ($7$) in \name}.
%  Since we have no access to such a trace, we
%  created such such a trace by removing all coflows with 7 or fewer lows.
Fig.~\ref{fig:sim:cctOthers:onlyWide} shows that \name continues
to perform well, reducing the average CCT by 1.54$\times$, 1.15$\times$, and
1.12$\times$ over Aalo, Aalo-Oracle, and SEBF, respectively.

%% \name performs good
%% for thin coflows (bin 1 and bin3). The good performance for thin and
%% small coflows (36\%) is because \name does right job in prioritizing
%% them. Becuase of the feature of prioritizing thin jobs bin-3 also see
%% good improvements.  \name also performs well for large and wide
%% coflows.  large and thin coflows name achieves speedup greater than 1
%% for 33\% of coflows in the bin. Poor performance for some of the
%% coflows in bin - 2 is because even if they are small they are being
%% probed for size estimation and this making them pay double penalty. \\

%% Overall \name speeds up more than 65\% of coflows, figure
%% ~\ref{figs:sim:speedUp} shows, the CDF of individual CCT improvement under
%% \name as compared to Aalo.

\begin{figure}
\begin{minipage}{0.22\textwidth}
\includegraphics[width=1.0\textwidth, natwidth=610,natheight=642]{figs/binning.pdf} %done
\vspace{-0.3in}
\caption{Performance breakdown into bins shown in Table~\ref{table:sim:bin}.
}
\label{figs:speedup:bin}
\end{minipage}
\hfill
\begin{minipage}{0.25\textwidth} % -- This is a testbed figure.
\centering
\includegraphics[width=1.0\linewidth, natwidth=610,natheight=642]{figs/eval/ATC19-testbed-speedup-jct-cct.pdf}
\vspace{-0.3in}
\caption{[Testbed] Distribution of speedup in CCT and JCT in \name using the FB trace.}
\label{fig:eval:jct-cct-speedUp}
\end{minipage}
\vspace{-0.1in}
\end{figure} 

\begin{table}
%\vspace{-0.1in}
  \caption{Bins based on total coflow size and width (number of flows). The
numbers in brackets denote the fraction of coflows in that bin.}
%\vspace{-0.1in}
  \label{table:sim:bin}
  \centering
      {\small
	\begin{tabular}{|c|c|c|c|c|} 
	  \hline
	  & width $\leq$ 7 (thin) & width $>$ 7 (wide) \\
%          & (thin) & (wide)\\
	  \hline
	  size $\leq$ 100MB (small) & bin-1 (44.3\%) & bin-2 (24.1\%) \\
	  \hline
	  size $>$ 100MB (large) & bin-3 (4.5\%) & bin-4 (27.1\%) \\
	  \hline
	\end{tabular}
      }
\vspace{-0.15in}
\end{table}

%% \begin{figure}
%%   \includegraphics[width=\textwidth]{figs/speedUp-CDF.eps} %done
%%   \caption{Speedup in CCT in \name}
%%   \label{figs:sim:speedUp}
%% \end{figure}

%\vspace{-0.1in}
\subsection{Robustness to coflow data skew}
\label{sec:sim:skew}
\begin{figure} 
\vspace{-0.2in}
\centering
\subfigure[\vspace{-0.2in}Using 5 Low-skew-filtered traces.]
{
%\vspace{-0.2in}
\includegraphics[width=0.48\linewidth, natwidth=610,natheight=642]{figs/PerformanceCompareLowSkewFilter.pdf}	% done
\hspace{-0.15in}
\label{fig:sim:cctOthers:skew:lowSkewFilter}
}
\subfigure[\vspace{-0.2in}Using the Mantri-like trace.]
{
\includegraphics[width=0.48\linewidth, natwidth=610,natheight=642]{figs/PerformanceCompareMantri.pdf}	% done
\hspace{-0.15in}
\label{fig:sim:cctOthers:skew:mantri}
} 
\vspace{-0.1in}
\caption{CCT speedup using \name compared to using other coflow schedulers on
  traces with different skew.
  In Fig.~\ref{fig:sim:cctOthers:skew:lowSkewFilter},
  % shows improvements of \name over Aalo only
the x-axis denotes the minimum skew in 
the 5 Low-skew-filtered traces.
%   \addaj{Y-axis denotes speedup i.e. ratio of CCTs}
}
\vspace{-0.2in}
\label{fig:sim:cctOthers:skew}
\end{figure}


%\begin{figure}[tp] 
%\centering
%\vspace{-0.1in}
%% \subfigure[Mix of thin and wide coflows] {
%\includegraphics[width=0.23\linewidth]{figs/PerformanceCompareLowSkewFilter.pdf}	% done
%%  \label{fig:sim:cctOthers:all}
%\\
%\vspace{-0.1in}
%(a)
%CCT improvement of \name over Aalo
%using Low-skew-filtered traces. The x-axis denotes the
%minimum skew in the five traces.
%%  The figure shows speedups and average CCT
%\\
%\includegraphics[width=0.23\linewidth]{figs/PerformanceCompareMantri.pdf}	% done
%%\label{fig:sim:skewedTrace:mantri}
%\\
%\vspace{-0.1in}
%(b)
%% Trace with skew across map tasks similar to what is described in
%Using the Mantri-like trace.
%\vspace{0.1in}
%\caption{CCT speedup using \name as compared to other Aalo on skewed traces.
%\updated {06/13/2018} 
%% The Y-axis denotes the improvement in speedups and average cct.
%} 
%\label{fig:sim:skewedTrace}
%\vspace{-0.1in} 
%\end{figure}

\if 0
Previous work~\cite{varys:sigcomm14} has shown that most coflows in large
production clusters have no skew, a majority among the remaining have very low
skew, and only very few of them have high skew.
% Since \name's approach of
% sampling few flows for estimating size benefits coflows with low skew
Nevertheless, to rigorously evaluate \name, 
\fi
Next, we evaluate \name's robustness to flow size skew
by comparing it against Aalo using {traces with varying degrees of skew}.
First, we evaluate \name using the Mantri-like trace. 
Fig.~\ref{fig:sim:cctOthers:skew:mantri} shows that
\name consistently outperforms prior-art coflow schedulers.
{In particular, \name reduces the average CCT by
1.36x compared to Aalo}.
%
Second, we evaluate \name using the Low-skew-filtered traces which have
low skew coflows filtered out.  Fig.~\ref{fig:sim:cctOthers:skew:lowSkewFilter}
shows that \name performs better than Aalo even with highly skewed
traces and reduces the average CCT by 1.45$\times$, 1.44$\times$,
1.44$\times$, 1.40$\times$ and 1.38$\times$ for the five
Low-skew-filtered traces containing coflows with skew of at least 1,
2, 3, 4 and 5, respectively.

\if 0
\paragraph{Can \name handle extreme skew?}
  \addaj{To stress test \name's performance under high skew we derived 2 more traces similar to Mantri-like trace with 2$\times$(3$\times$) the skew as mentioned in the Mantri\cite{mantri:OSDI2010}. \name achieves average CCT speedupof 1.18$\times$(0.98$\times$) and P50 speedup in individual CCTs is 1.38$\times$(1.48$\times$)}
  \fi

{\input sensitivity }

